Hashing-based Non-Maximum Suppression for Crowded Object Detection

In this paper, we propose an algorithm, named hashing-based non-maximum suppression (HNMS) to efficiently suppress the non-maximum boxes for object detection. Non-maximum suppression (NMS) is an essential component to suppress the boxes at closely located locations with similar shapes. The time cost tends to be huge when the number of boxes becomes large, especially for crowded scenes. The basic idea of HNMS is to firstly map each box to a discrete code (hash cell) and then remove the boxes with lower confidences if they are in the same cell. Considering the intersection-over-union (IoU) as the metric, we propose a simple yet effective hashing algorithm, named IoUHash, which guarantees that the boxes within the same cell are close enough by a lower IoU bound. For two-stage detectors, we replace NMS in region proposal network with HNMS, and observe significant speed-up with comparable accuracy. For one-stage detectors, HNMS is used as a pre-filter to speed up the suppression with a large margin. Extensive experiments are conducted on CARPK, SKU-110K, CrowdHuman datasets to demonstrate the efficiency and effectiveness of HNMS. Code is released at \url{https://github.com/microsoft/hnms.git}.

==> table/cuda_retina_table.tex <==
\begin{table}
\centering
\caption{Experiment results on CARPK with Retina-R50-FPN. The columns of HNMS, NMS and Total represent the time cost in ms. Speed is for the total cost by HNMS and NMS.}
\label{tbl:retina_CARPK}
\begin{tabular}{c@{~}c@{~}c@{~~}c@{~~}c@{~~}c@{~~}c}
\toprule
 & $K$ & mAP & HNMS & NMS & Speed & Total\\
\midrule
NMS &  & 94.8 &  & $134.7\pm 12.7$ & 1x & $250.9\pm 17.4$\\
\midrule
\multirow{4}{*}{HNMS} & 1 & \textbf{95.3} & $0.9\pm 0.2$ & $33.1\pm 21.6$ & \textbf{3.96x} & $149.1\pm 26.4$\\
 & 2 & \textbf{95.3} & $1.4\pm 0.2$ & $18.4\pm 13.5$ & \textbf{6.80x} & $121.9\pm 17.1$\\
 & 3 & 95.2 & $2.5\pm 0.5$ & $19.5\pm 13.7$ & 6.12x & $142.1\pm 18.5$\\
 & 4 & 95.2 & $3.0\pm 0.5$ & $14.6\pm 9.0$ & 7.65x & $131.3\pm 20.1$\\
\bottomrule
\end{tabular}
\end{table}\begin{table}
\centering
\caption{Experiment results on SKU-110K with Retina-R50-FPN. The columns of HNMS, NMS and Total represent the time cost in ms. Speed is for the total cost by HNMS and NMS.}
\label{tbl:retina_SKU-110K}
\begin{tabular}{c@{~}c@{~}c@{~~}c@{~~}c@{~~}c@{~~}c}
\toprule
 & $K$ & mAP & HNMS & NMS & Speed & Total\\
\midrule
NMS &  & \textbf{91.6} &  & $121.1\pm 15.4$ & \textbf{1x} & $217.9\pm 25.9$\\
\midrule
\multirow{4}{*}{HNMS} & 1 & \textbf{91.6} & $0.7\pm 0.1$ & $18.8\pm 7.1$ & \textbf{6.21x} & $115.8\pm 15.7$\\
 & 2 & \textbf{91.6} & $1.4\pm 0.2$ & $14.0\pm 3.6$ & \textbf{7.86x} & $111.3\pm 10.9$\\
 & 3 & 91.5 & $2.1\pm 0.3$ & $11.3\pm 2.9$ & 9.04x & $109.0\pm 9.9$\\
 & 4 & 91.5 & $2.8\pm 0.4$ & $10.9\pm 3.2$ & 8.84x & $111.4\pm 11.6$\\
\bottomrule
\end{tabular}
\end{table}\begin{table}
\centering
\caption{Experiment results on CrowdHuman with Retina-R50-FPN. The columns of HNMS, NMS and Total represent the time cost in ms. Speed is for the total cost by HNMS and NMS.}
\label{tbl:retina_CrowdHuman}
\begin{tabular}{c@{~}c@{~}c@{~~}c@{~~}c@{~~}c@{~~}c}
\toprule
 & $K$ & mAP & HNMS & NMS & Speed & Total\\
\midrule
NMS &  & 77.7 &  & $139.1\pm 19.1$ & 1x & $252.3\pm 25.3$\\
\midrule
\multirow{4}{*}{HNMS} & 1 & \textbf{77.8} & $0.9\pm 0.4$ & $66.5\pm 15.2$ & \textbf{2.06x} & $179.3\pm 21.4$\\
 & 2 & 77.6 & $1.7\pm 0.3$ & $36.3\pm 16.6$ & 3.66x & $152.8\pm 20.6$\\
 & 3 & 77.5 & $2.5\pm 0.5$ & $25.1\pm 8.6$ & 5.04x & $140.6\pm 16.7$\\
 & 4 & 77.4 & $3.3\pm 0.5$ & $22.6\pm 9.1$ & 5.37x & $142.4\pm 15.9$\\
\bottomrule
\end{tabular}
\end{table}

==> table/cuda_rpn.tex <==
\begin{table}
\centering
\caption{Experiment results on CARPK with Faster-RCNN-R50-FPN. The columns of RPN-NMS and Total represent the time cost in ms. Speed is for RPN-NMS.}
\label{tbl:faster_CARPK}
\begin{tabular}{c@{~}c@{~}c@{~~}c@{~~}c@{~~}c}
\toprule
 & $K$ & mAP & RPN-NMS & Speed & Total\\
\midrule
NMS &  & 96.9 & $27.2\pm 2.0$ & 1x & $149.0\pm 5.9$\\
\midrule
\multirow{4}{*}{HNMS} & 1 & \textbf{97.1} & $6.5\pm 1.0$ & \textbf{4.18x} & $132.8\pm 9.1$\\
 & 2 & \textbf{97.1} & $9.3\pm 1.2$ & \textbf{2.92x} & $137.9\pm 8.0$\\
 & 3 & 97.0 & $11.2\pm 1.5$ & 2.43x & $136.9\pm 10.7$\\
 & 4 & 96.9 & $13.2\pm 1.7$ & 2.06x & $136.2\pm 9.9$\\
\bottomrule
\end{tabular}
\end{table}\begin{table}
\centering
\caption{Experiment results on SKU-110K with Faster-RCNN-R50-FPN. The columns of RPN-NMS and Total represent the time cost in ms. Speed is for RPN-NMS.}
\label{tbl:faster_SKU-110K}
\begin{tabular}{c@{~}c@{~}c@{~~}c@{~~}c@{~~}c}
\toprule
 & $K$ & mAP & RPN-NMS & Speed & Total\\
\midrule
NMS &  & \textbf{90.5} & $32.2\pm 3.7$ & \textbf{1x} & $133.7\pm 10.1$\\
\midrule
\multirow{4}{*}{HNMS} & 1 & 89.8 & $5.9\pm 0.6$ & 5.46x & $101.4\pm 6.7$\\
 & 2 & 90.4 & $8.6\pm 0.6$ & 3.74x & $103.8\pm 6.6$\\
 & 3 & \textbf{90.5} & $11.4\pm 1.3$ & \textbf{2.82x} & $107.8\pm 8.9$\\
 & 4 & \textbf{90.5} & $17.1\pm 1.9$ & \textbf{1.88x} & $101.4\pm 8.1$\\
\bottomrule
\end{tabular}
\end{table}\begin{table}
\centering
\caption{Experiment results on CrowdHuman with Faster-RCNN-R50-FPN. The columns of RPN-NMS and Total represent the time cost in ms. Speed is for RPN-NMS.}
\label{tbl:faster_CrowdHuman}
\begin{tabular}{c@{~}c@{~}c@{~~}c@{~~}c@{~~}c}
\toprule
 & $K$ & mAP & RPN-NMS & Speed & Total\\
\midrule
NMS &  & \textbf{82.1} & $27.3\pm 4.3$ & \textbf{1x} & $148.8\pm 11.6$\\
\midrule
\multirow{4}{*}{HNMS} & 1 & 81.8 & $6.3\pm 0.8$ & 4.33x & $101.8\pm 6.4$\\
 & 2 & 82.0 & $10.4\pm 1.3$ & 2.62x & $114.4\pm 10.0$\\
 & 3 & 82.0 & $12.6\pm 0.8$ & 2.17x & $110.6\pm 5.3$\\
 & 4 & \textbf{82.1} & $15.4\pm 0.9$ & \textbf{1.77x} & $113.7\pm 4.5$\\
\bottomrule
\end{tabular}
\end{table}

==> table/device_retina_table.tex <==
\begin{table}
\centering
\caption{Experiment results on CARPK with Retina-R50-FPN. The columns of HNMS, NMS and Total represent the time cost in ms. Speed is for the total cost by HNMS and NMS.}
\label{tbl:retina_CARPK}
\begin{tabular}{c@{~~}c@{~~}c@{~~~}c@{~}c@{~}c@{~}c@{~~~}c@{~}c@{~}c@{~}c}
\toprule
 &  &  & \multicolumn{4}{c}{CPU} & \multicolumn{4}{c}{GPU}\\
\cmidrule(lr){4-7}
\cmidrule(lr){8-11}
 & $K$ & mAP & HNMS & NMS & Speed & Total & HNMS & NMS & Speed & Total\\
\midrule
NMS &  & 94.8 &  & 260.9 & 1x & 2071.1 &  & 134.7 & 1x & 250.9\\
\midrule
 & 1 & \textbf{95.3} & 23.6 & 194.2 & \textbf{1.2x} & 1761.9 & 0.9 & 33.1 & \textbf{4.0x} & 149.1\\
HNMS & 2 & \textbf{95.3} & 34.0 & 161.7 & \textbf{1.3x} & 1762.6 & 1.4 & 18.4 & \textbf{6.8x} & 121.9\\
+NMS & 3 & 95.2 & 46.1 & 140.4 & 1.4x & 1794.6 & 2.5 & 19.5 & 6.1x & 142.1\\
 & 4 & 95.2 & 51.4 & 122.4 & 1.5x & 1732.6 & 3.0 & 14.6 & 7.7x & 131.3\\
\bottomrule
\end{tabular}
\end{table}\begin{table}
\centering
\caption{Experiment results on SKU-110K with Retina-R50-FPN. The columns of HNMS, NMS and Total represent the time cost in ms. Speed is for the total cost by HNMS and NMS.}
\label{tbl:retina_SKU-110K}
\begin{tabular}{c@{~~}c@{~~}c@{~~~}c@{~}c@{~}c@{~}c@{~~~}c@{~}c@{~}c@{~}c}
\toprule
 &  &  & \multicolumn{4}{c}{CPU} & \multicolumn{4}{c}{GPU}\\
\cmidrule(lr){4-7}
\cmidrule(lr){8-11}
 & $K$ & mAP & HNMS & NMS & Speed & Total & HNMS & NMS & Speed & Total\\
\midrule
NMS &  & \textbf{91.6} &  & 185.2 & \textbf{1x} & 1640.9 &  & 121.1 & \textbf{1x} & 217.9\\
\midrule
 & 1 & \textbf{91.6} & 19.4 & 124.5 & \textbf{1.3x} & 1576.3 & 0.7 & 18.8 & \textbf{6.2x} & 115.8\\
HNMS & 2 & \textbf{91.6} & 33.9 & 104.2 & \textbf{1.3x} & 1567.6 & 1.4 & 14.0 & \textbf{7.9x} & 111.3\\
+NMS & 3 & 91.5 & 42.7 & 88.2 & 1.4x & 1571.8 & 2.1 & 11.3 & 9.1x & 109.0\\
 & 4 & 91.5 & 50.3 & 81.0 & 1.4x & 1531.5 & 2.8 & 10.9 & 8.9x & 111.4\\
\bottomrule
\end{tabular}
\end{table}\begin{table}
\centering
\caption{Experiment results on CrowdHuman with Retina-R50-FPN. The columns of HNMS, NMS and Total represent the time cost in ms. Speed is for the total cost by HNMS and NMS.}
\label{tbl:retina_CrowdHuman}
\begin{tabular}{c@{~~}c@{~~}c@{~~~}c@{~}c@{~}c@{~}c@{~~~}c@{~}c@{~}c@{~}c}
\toprule
 &  &  & \multicolumn{4}{c}{CPU} & \multicolumn{4}{c}{GPU}\\
\cmidrule(lr){4-7}
\cmidrule(lr){8-11}
 & $K$ & mAP & HNMS & NMS & Speed & Total & HNMS & NMS & Speed & Total\\
\midrule
NMS &  & 77.7 &  & 327.8 & 1x & 1870.9 &  & 143.9 & 1x & 260.5\\
\midrule
 & 1 & \textbf{77.8} & 25.0 & 268.7 & \textbf{1.1x} & 1653.4 & 0.9 & 65.1 & \textbf{2.2x} & 182.1\\
HNMS & 2 & 77.6 & 42.2 & 234.5 & 1.2x & 1837.4 & 1.6 & 39.4 & 3.5x & 151.3\\
+NMS & 3 & 77.5 & 56.8 & 216.4 & 1.2x & 1858.9 & 2.3 & 29.4 & 4.5x & 139.1\\
 & 4 & 77.4 & 66.2 & 193.5 & 1.3x & 1841.9 & 3.2 & 24.3 & 5.2x & 142.2\\
\bottomrule
\end{tabular}
\end{table}

==> table/device_rpn.tex <==
\begin{table}
\centering
\caption{Experiment results on CARPK with Faster-RCNN-R50-FPN. The columns of RPN-NMS and Total represent the time cost in ms. Speed is for RPN-NMS.}
\label{tbl:faster_CARPK}
\begin{tabular}{c@{~~}c@{~~}c@{~~~}ccc@{~~~}ccc}
\toprule
 &  &  & \multicolumn{3}{c}{CPU} & \multicolumn{3}{c}{GPU}\\
\cmidrule(lr){4-6}
\cmidrule(lr){7-9}
 & $K$ & mAP & RPN-NMS & Speed & Total & RPN-NMS & Speed & Total\\
\midrule
NMS &  & 96.9 & $223.3\pm 36.5$ & 1x & 3935.7 & $27.2\pm 2.0$ & 1x & 149.0\\
\midrule
\multirow{4}{*}{HNMS} & 1 & \textbf{97.1} & $30.3\pm 5.4$ & \textbf{7.4x} & 3665.6 & $6.5\pm 1.0$ & \textbf{4.2x} & 132.8\\
 & 2 & \textbf{97.1} & $49.0\pm 6.5$ & \textbf{4.6x} & 3571.5 & $9.3\pm 1.2$ & \textbf{2.9x} & 137.9\\
 & 3 & 97.0 & $52.3\pm 7.6$ & 4.3x & 3790.5 & $11.2\pm 1.5$ & 2.4x & 136.9\\
 & 4 & 96.9 & $68.8\pm 9.6$ & 3.2x & 3790.6 & $13.2\pm 1.7$ & 2.1x & 136.2\\
\bottomrule
\end{tabular}
\end{table}\begin{table}
\centering
\caption{Experiment results on SKU-110K with Faster-RCNN-R50-FPN. The columns of RPN-NMS and Total represent the time cost in ms. Speed is for RPN-NMS.}
\label{tbl:faster_SKU-110K}
\begin{tabular}{c@{~~}c@{~~}c@{~~~}ccc@{~~~}ccc}
\toprule
 &  &  & \multicolumn{3}{c}{CPU} & \multicolumn{3}{c}{GPU}\\
\cmidrule(lr){4-6}
\cmidrule(lr){7-9}
 & $K$ & mAP & RPN-NMS & Speed & Total & RPN-NMS & Speed & Total\\
\midrule
NMS &  & \textbf{90.5} & $478.4\pm 64.4$ & \textbf{1x} & 2599.9 & $32.2\pm 3.7$ & \textbf{1x} & 133.7\\
\midrule
\multirow{4}{*}{HNMS} & 1 & 89.8 & $41.4\pm 5.8$ & 11.6x & 2191.5 & $5.9\pm 0.6$ & 5.5x & 101.4\\
 & 2 & 90.4 & $69.2\pm 7.4$ & 6.9x & 2220.2 & $8.6\pm 0.6$ & 3.7x & 103.8\\
 & 3 & \textbf{90.5} & $79.9\pm 11.8$ & \textbf{6.0x} & 2250.3 & $11.4\pm 1.3$ & \textbf{2.8x} & 107.8\\
 & 4 & \textbf{90.5} & $102.6\pm 11.8$ & \textbf{4.7x} & 2239.9 & $17.1\pm 1.9$ & \textbf{1.9x} & 101.4\\
\bottomrule
\end{tabular}
\end{table}\begin{table}
\centering
\caption{Experiment results on CrowdHuman with Faster-RCNN-R50-FPN. The columns of RPN-NMS and Total represent the time cost in ms. Speed is for RPN-NMS.}
\label{tbl:faster_CrowdHuman}
\begin{tabular}{c@{~~}c@{~~}c@{~~~}ccc@{~~~}ccc}
\toprule
 &  &  & \multicolumn{3}{c}{CPU} & \multicolumn{3}{c}{GPU}\\
\cmidrule(lr){4-6}
\cmidrule(lr){7-9}
 & $K$ & mAP & RPN-NMS & Speed & Total & RPN-NMS & Speed & Total\\
\midrule
NMS &  & \textbf{82.1} & $307.9\pm 48.4$ & \textbf{1x} & 3643.5 & $27.3\pm 4.3$ & \textbf{1x} & 148.8\\
\midrule
\multirow{4}{*}{HNMS} & 1 & 81.8 & $38.9\pm 6.6$ & 7.9x & 3379.8 & $6.3\pm 0.8$ & 4.3x & 101.8\\
 & 2 & 82.0 & $53.8\pm 6.7$ & 5.7x & 3584.5 & $10.4\pm 1.3$ & 2.6x & 114.4\\
 & 3 & 82.0 & $64.1\pm 9.4$ & 4.8x & 3530.9 & $12.6\pm 0.8$ & 2.2x & 110.6\\
 & 4 & \textbf{82.1} & $73.0\pm 10.9$ & \textbf{4.2x} & 3434.4 & $15.4\pm 0.9$ & \textbf{1.8x} & 113.7\\
\bottomrule
\end{tabular}
\end{table}

==> table/retina.bak.tex <==
\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RPN-Rerank & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $27.8\pm 6.4$ &  & $1696.2\pm 74.2$ &  & CARPK & 91.9 & 2000\\
$6.2\pm 1.2$ & $16.5\pm 4.7$ & $8.5\pm 3.6$ & $1568.7\pm 156.4$ & ret0.6/1 & CARPK & 91.5 & 2000\\
$8.7\pm 1.1$ & $28.8\pm 6.0$ & $17.6\pm 5.2$ & $1661.8\pm 53.5$ & ret0.7/1 & CARPK & 91.6 & 2000\\
 &  &  &  & ret0.73/1 & CARPK & 91.8 & 2000\\
$8.0\pm 1.6$ & $30.4\pm 8.8$ & $20.4\pm 7.4$ & $1597.2\pm 140.6$ & ret0.8/1 & CARPK & 91.8 & 2000\\
 &  &  &  & ret0.6/2 & CARPK & 91.1 & 2000\\
$11.3\pm 2.7$ & $24.2\pm 6.6$ & $11.1\pm 3.8$ & $1571.9\pm 129.1$ & ret0.7/2 & CARPK & 91.5 & 2000\\
 &  &  &  & ret0.73/2 & CARPK & 91.7 & 2000\\
$12.9\pm 2.4$ & $33.1\pm 7.5$ & $18.5\pm 5.5$ & $1490.5\pm 192.8$ & ret0.8/2 & CARPK & 91.8 & 2000\\
 &  &  &  & ret0.6/3 & CARPK & 91.0 & 2000\\
$13.8\pm 2.4$ & $24.8\pm 5.4$ & $9.3\pm 3.3$ & $1547.3\pm 145.7$ & ret0.7/3 & CARPK & 91.4 & 2000\\
 &  &  &  & ret0.73/3 & CARPK & 91.6 & 2000\\
$18.2\pm 3.3$ & $38.3\pm 8.4$ & $18.2\pm 5.7$ & $1523.1\pm 107.5$ & ret0.8/3 & CARPK & 91.7 & 2000\\
 &  &  &  & ret0.6/4 & CARPK & 90.8 & 2000\\
$16.8\pm 3.5$ & $26.8\pm 6.6$ & $8.4\pm 3.2$ & $1540.0\pm 168.3$ & ret0.7/4 & CARPK & 91.3 & 2000\\
 &  &  &  & ret0.73/4 & CARPK & 91.5 & 2000\\
$22.0\pm 3.9$ & $40.8\pm 8.7$ & $17.1\pm 5.4$ & $1582.3\pm 138.1$ & ret0.8/4 & CARPK & 91.7 & 2000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RPN-Rerank & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $45.0\pm 15.9$ &  & $1709.8\pm 108.0$ &  & CARPK & 93.1 & 3000\\
$8.3\pm 1.6$ & $24.7\pm 8.9$ & $14.1\pm 7.7$ & $1544.5\pm 135.2$ & ret0.6/1 & CARPK & 92.7 & 3000\\
$11.8\pm 1.6$ & $45.8\pm 13.7$ & $30.7\pm 12.4$ & $1670.4\pm 60.3$ & ret0.7/1 & CARPK & 92.9 & 3000\\
 &  &  &  & ret0.73/1 & CARPK & 93.5 & 3000\\
$10.7\pm 2.0$ & $48.7\pm 17.8$ & $35.3\pm 16.3$ & $1581.8\pm 158.6$ & ret0.8/1 & CARPK & 93.0 & 3000\\
 &  &  &  & ret0.6/2 & CARPK & 92.4 & 3000\\
$14.3\pm 2.7$ & $34.9\pm 11.6$ & $18.6\pm 9.3$ & $1596.5\pm 155.4$ & ret0.7/2 & CARPK & 92.8 & 3000\\
 &  &  &  & ret0.73/2 & CARPK & 92.9 & 3000\\
$18.5\pm 3.7$ & $54.9\pm 19.2$ & $34.0\pm 16.3$ & $1587.4\pm 99.7$ & ret0.8/2 & CARPK & 93.0 & 3000\\
 &  &  &  & ret0.6/3 & CARPK & 92.2 & 3000\\
$21.1\pm 3.8$ & $41.0\pm 11.4$ & $17.5\pm 8.2$ & $1686.2\pm 110.6$ & ret0.7/3 & CARPK & 92.7 & 3000\\
 &  &  &  & ret0.73/3 & CARPK & 92.8 & 3000\\
$24.6\pm 4.7$ & $58.8\pm 17.1$ & $31.9\pm 13.9$ & $1567.9\pm 122.8$ & ret0.8/3 & CARPK & 92.9 & 3000\\
 &  &  &  & ret0.6/4 & CARPK & 92.0 & 3000\\
$24.1\pm 5.9$ & $42.0\pm 14.7$ & $15.6\pm 9.0$ & $1652.7\pm 138.4$ & ret0.7/4 & CARPK & 92.6 & 3000\\
 &  &  &  & ret0.73/4 & CARPK & 92.7 & 3000\\
$29.9\pm 5.4$ & $63.0\pm 17.5$ & $30.7\pm 13.2$ & $1592.9\pm 127.8$ & ret0.8/4 & CARPK & 92.9 & 3000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RPN-Rerank & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $121.1\pm 59.3$ &  & $1785.7\pm 111.2$ &  & CARPK & 94.5 & 6000\\
$15.8\pm 3.3$ & $59.4\pm 30.2$ & $39.6\pm 28.0$ & $1614.1\pm 114.6$ & ret0.6/1 & CARPK & 94.3 & 6000\\
$19.4\pm 2.6$ & $109.8\pm 50.4$ & $85.5\pm 49.0$ & $1722.9\pm 70.8$ & ret0.7/1 & CARPK & 94.3 & 6000\\
 &  &  &  & ret0.73/1 & CARPK & 94.4 & 6000\\
$19.0\pm 4.0$ & $127.4\pm 59.1$ & $104.5\pm 57.3$ & $1667.4\pm 165.5$ & ret0.8/1 & CARPK & 94.4 & 6000\\
 &  &  &  & ret0.6/2 & CARPK & 93.9 & 6000\\
$25.1\pm 4.4$ & $83.3\pm 40.4$ & $54.5\pm 37.3$ & $1638.0\pm 158.0$ & ret0.7/2 & CARPK & 94.2 & 6000\\
 &  &  &  & ret0.73/2 & CARPK & 94.3 & 6000\\
$30.8\pm 5.7$ & $131.1\pm 60.4$ & $97.0\pm 56.5$ & $1604.0\pm 191.6$ & ret0.8/2 & CARPK & 94.4 & 6000\\
 &  &  &  & ret0.6/3 & CARPK & 93.7 & 6000\\
$34.3\pm 6.9$ & $87.1\pm 42.0$ & $48.7\pm 36.5$ & $1705.8\pm 108.1$ & ret0.7/3 & CARPK & 94.1 & 6000\\
 &  &  &  & ret0.73/3 & CARPK & 94.2 & 6000\\
$42.2\pm 8.7$ & $140.8\pm 63.6$ & $95.1\pm 57.1$ & $1621.9\pm 164.1$ & ret0.8/3 & CARPK & 94.4 & 6000\\
 &  &  &  & ret0.6/4 & CARPK & 93.5 & 6000\\
$37.5\pm 9.1$ & $80.3\pm 37.4$ & $39.4\pm 29.2$ & $1567.3\pm 166.9$ & ret0.7/4 & CARPK & 94.1 & 6000\\
 &  &  &  & ret0.73/4 & CARPK & 94.2 & 6000\\
$51.2\pm 11.2$ & $145.8\pm 63.8$ & $91.1\pm 54.4$ & $1684.4\pm 160.1$ & ret0.8/4 & CARPK & 94.4 & 6000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RPN-Rerank & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $260.9\pm 104.8$ &  & $2071.1\pm 230.5$ &  & CARPK & 94.8 & 9000\\
$23.3\pm 5.4$ & $111.6\pm 62.9$ & $82.8\pm 58.6$ & $1619.4\pm 145.3$ & ret0.6/1 & CARPK & 94.6 & 9000\\
$25.7\pm 4.2$ & $208.0\pm 89.1$ & $176.4\pm 87.1$ & $1827.5\pm 146.9$ & ret0.7/1 & CARPK & 94.7 & 9000\\
$23.6\pm 4.9$ & $223.2\pm 104.0$ & $194.2\pm 100.9$ & $1761.9\pm 149.7$ & ret0.73/1 & CARPK & 95.3 & 9000\\
$27.6\pm 5.1$ & $245.5\pm 101.5$ & $212.4\pm 99.7$ & $1836.4\pm 152.7$ & ret0.75/1 & CARPK & 94.8 & 9000\\
$27.9\pm 6.2$ & $274.8\pm 120.4$ & $241.5\pm 115.7$ & $1824.2\pm 195.7$ & ret0.8/1 & CARPK & 94.8 & 9000\\
 &  &  &  & ret0.6/2 & CARPK & 94.3 & 9000\\
$39.3\pm 8.0$ & $176.9\pm 81.9$ & $132.3\pm 75.8$ & $1739.6\pm 151.7$ & ret0.7/2 & CARPK & 94.7 & 9000\\
$34.0\pm 6.4$ & $200.1\pm 93.7$ & $161.7\pm 88.6$ & $1762.6\pm 187.2$ & ret0.73/2 & CARPK & 95.3 & 9000\\
 &  &  &  & ret0.75/2 & CARPK & 94.8 & 9000\\
$46.1\pm 8.1$ & $282.2\pm 112.5$ & $230.9\pm 107.7$ & $1817.3\pm 182.7$ & ret0.8/2 & CARPK & 94.8 & 9000\\
 &  &  &  & ret0.6/3 & CARPK & 94.1 & 9000\\
$45.9\pm 9.4$ & $153.9\pm 74.1$ & $103.2\pm 65.8$ & $1748.8\pm 140.9$ & ret0.7/3 & CARPK & 94.6 & 9000\\
$46.1\pm 8.5$ & $191.3\pm 86.7$ & $140.4\pm 80.2$ & $1794.6\pm 108.5$ & ret0.73/3 & CARPK & 95.2 & 9000\\
 &  &  &  & ret0.75/3 & CARPK & 94.7 & 9000\\
$59.6\pm 12.1$ & $280.9\pm 120.2$ & $216.6\pm 111.4$ & $1807.2\pm 198.1$ & ret0.8/3 & CARPK & 94.8 & 9000\\
 &  &  &  & ret0.6/4 & CARPK & 94.0 & 9000\\
$57.8\pm 13.4$ & $158.8\pm 74.4$ & $95.7\pm 62.6$ & $1718.8\pm 133.6$ & ret0.7/4 & CARPK & 94.5 & 9000\\
$51.4\pm 8.4$ & $178.3\pm 74.7$ & $122.4\pm 67.8$ & $1732.6\pm 129.7$ & ret0.73/4 & CARPK & 95.2 & 9000\\
 &  &  &  & ret0.75/4 & CARPK & 94.7 & 9000\\
$78.0\pm 15.0$ & $296.2\pm 117.5$ & $213.1\pm 105.8$ & $1852.7\pm 170.1$ & ret0.8/4 & CARPK & 94.7 & 9000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RPN-Rerank & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $286.8\pm 113.1$ &  & $1885.2\pm 163.7$ &  & CARPK & 95.4 & 10000\\
$18.5\pm 3.3$ & $124.4\pm 64.8$ & $100.4\pm 63.0$ & $1695.5\pm 166.4$ & ret0.6/1 & CARPK & 95.3 & 10000\\
$19.2\pm 3.1$ & $220.7\pm 103.0$ & $196.8\pm 101.7$ & $1758.9\pm 172.1$ & ret0.7/1 & CARPK & 95.4 & 10000\\
$19.8\pm 3.3$ & $249.0\pm 110.5$ & $224.3\pm 109.0$ & $1801.0\pm 171.7$ & ret0.73/1 & CARPK & 95.4 & 10000\\
$21.4\pm 3.9$ & $272.1\pm 115.6$ & $245.7\pm 113.1$ & $1931.7\pm 153.9$ & ret0.75/1 & CARPK & 95.4 & 10000\\
$21.5\pm 3.5$ & $306.3\pm 125.2$ & $279.4\pm 124.1$ & $1876.7\pm 173.9$ & ret0.8/1 & CARPK & 95.4 & 10000\\
$23.7\pm 4.5$ & $84.9\pm 39.2$ & $56.0\pm 36.1$ & $1602.6\pm 133.5$ & ret0.6/2 & CARPK & 95.0 & 10000\\
$28.8\pm 4.7$ & $183.5\pm 85.0$ & $149.7\pm 82.3$ & $1745.8\pm 129.2$ & ret0.7/2 & CARPK & 95.3 & 10000\\
$31.6\pm 6.5$ & $229.2\pm 109.9$ & $192.7\pm 105.6$ & $1790.5\pm 167.1$ & ret0.73/2 & CARPK & 95.3 & 10000\\
$35.2\pm 6.6$ & $248.7\pm 106.7$ & $208.3\pm 102.3$ & $1973.5\pm 145.4$ & ret0.75/2 & CARPK & 95.4 & 10000\\
$36.2\pm 6.9$ & $303.7\pm 129.6$ & $262.2\pm 124.9$ & $1923.0\pm 141.0$ & ret0.8/2 & CARPK & 95.4 & 10000\\
$27.0\pm 5.8$ & $73.1\pm 31.6$ & $41.3\pm 26.8$ & $1611.2\pm 164.1$ & ret0.6/3 & CARPK & 94.8 & 10000\\
$36.3\pm 7.0$ & $166.7\pm 80.3$ & $125.5\pm 74.8$ & $1742.4\pm 160.4$ & ret0.7/3 & CARPK & 95.2 & 10000\\
$38.7\pm 8.3$ & $207.4\pm 97.2$ & $163.7\pm 90.1$ & $1759.2\pm 149.3$ & ret0.73/3 & CARPK & 95.3 & 10000\\
 &  &  &  & ret0.75/3 & CARPK & 95.3 & 10000\\
 &  &  &  & ret0.8/3 & CARPK & 94.8 & 10000\\
$32.8\pm 6.3$ & $74.6\pm 27.1$ & $36.6\pm 22.1$ & $1691.5\pm 122.4$ & ret0.6/4 & CARPK & 94.6 & 10000\\
$42.6\pm 7.0$ & $155.0\pm 71.8$ & $107.7\pm 66.4$ & $1701.4\pm 163.5$ & ret0.7/4 & CARPK & 95.2 & 10000\\
$48.9\pm 10.9$ & $208.3\pm 91.5$ & $154.0\pm 82.3$ & $1824.8\pm 134.7$ & ret0.73/4 & CARPK & 95.2 & 10000\\
 &  &  &  & ret0.75/4 & CARPK & 95.3 & 10000\\
 &  &  &  & ret0.8/4 & CARPK & 94.8 & 10000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RPN-Rerank & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $401.7\pm 150.8$ &  & $2037.4\pm 159.6$ &  & CARPK & 94.9 & 12000\\
$24.9\pm 3.8$ & $167.0\pm 74.8$ & $136.3\pm 73.1$ & $1678.2\pm 158.0$ & ret0.6/1 & CARPK & 94.8 & 12000\\
$31.2\pm 5.1$ & $313.1\pm 128.9$ & $275.6\pm 126.2$ & $1934.2\pm 146.9$ & ret0.7/1 & CARPK & 94.9 & 12000\\
 &  &  &  & ret0.73/1 & CARPK & 94.9 & 12000\\
$31.5\pm 4.7$ & $404.0\pm 158.5$ & $366.5\pm 156.6$ & $1932.9\pm 207.5$ & ret0.8/1 & CARPK & 94.9 & 12000\\
 &  &  &  & ret0.6/2 & CARPK & 94.5 & 12000\\
$43.3\pm 7.5$ & $257.4\pm 111.1$ & $208.8\pm 105.1$ & $1828.3\pm 202.8$ & ret0.7/2 & CARPK & 94.8 & 12000\\
 &  &  &  & ret0.73/2 & CARPK & 94.8 & 12000\\
$55.6\pm 9.6$ & $410.3\pm 157.8$ & $349.0\pm 152.0$ & $2013.9\pm 218.7$ & ret0.8/2 & CARPK & 94.9 & 12000\\
 &  &  &  & ret0.6/3 & CARPK & 94.3 & 12000\\
$57.2\pm 12.4$ & $240.5\pm 103.3$ & $177.9\pm 93.2$ & $1817.1\pm 175.1$ & ret0.7/3 & CARPK & 94.7 & 12000\\
 &  &  &  & ret0.73/3 & CARPK & 94.8 & 12000\\
$71.3\pm 12.6$ & $410.2\pm 161.9$ & $333.6\pm 152.7$ & $1980.3\pm 241.6$ & ret0.8/3 & CARPK & 94.9 & 12000\\
 &  &  &  & ret0.6/4 & CARPK & 94.1 & 12000\\
$66.3\pm 13.9$ & $231.9\pm 96.7$ & $160.1\pm 84.7$ & $1773.0\pm 224.9$ & ret0.7/4 & CARPK & 94.7 & 12000\\
 &  &  &  & ret0.73/4 & CARPK & 94.8 & 12000\\
$90.5\pm 17.2$ & $422.8\pm 168.3$ & $326.9\pm 155.9$ & $1967.4\pm 236.7$ & ret0.8/4 & CARPK & 94.9 & 12000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RPN-Rerank & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $19.6\pm 8.2$ &  & $1642.9\pm 180.5$ &  & human & 76.8 & 2000\\
 &  &  &  & ret0.6/1 & human & 76.4 & 2000\\
$8.2\pm 1.6$ & $22.4\pm 8.5$ & $12.0\pm 7.1$ & $1655.7\pm 190.9$ & ret0.7/1 & human & 76.6 & 2000\\
 &  &  &  & ret0.73/1 & human & 76.4 & 2000\\
$8.8\pm 1.6$ & $27.9\pm 9.3$ & $17.0\pm 8.0$ & $1586.7\pm 208.9$ & ret0.8/1 & human & 76.7 & 2000\\
 &  &  &  & ret0.6/2 & human & 76.1 & 2000\\
$12.4\pm 2.7$ & $23.0\pm 7.3$ & $8.8\pm 4.9$ & $1626.6\pm 172.2$ & ret0.7/2 & human & 76.4 & 2000\\
 &  &  &  & ret0.73/2 & human & 76.3 & 2000\\
$16.2\pm 3.4$ & $33.0\pm 9.4$ & $15.0\pm 7.2$ & $1549.4\pm 189.3$ & ret0.8/2 & human & 76.7 & 2000\\
 &  &  &  & ret0.6/3 & human & 75.8 & 2000\\
$15.1\pm 3.3$ & $24.2\pm 7.0$ & $7.2\pm 4.0$ & $1602.6\pm 181.9$ & ret0.7/3 & human & 76.3 & 2000\\
 &  &  &  & ret0.73/3 & human & 76.3 & 2000\\
$20.8\pm 4.8$ & $36.1\pm 10.7$ & $13.6\pm 6.8$ & $1546.4\pm 189.6$ & ret0.8/3 & human & 76.6 & 2000\\
 &  &  &  & ret0.6/4 & human & 75.6 & 2000\\
$17.8\pm 3.9$ & $25.9\pm 7.1$ & $6.4\pm 3.5$ & $1512.4\pm 201.9$ & ret0.7/4 & human & 76.3 & 2000\\
 &  &  &  & ret0.73/4 & human & 76.2 & 2000\\
$27.0\pm 5.2$ & $42.6\pm 10.8$ & $13.7\pm 6.8$ & $1598.2\pm 188.5$ & ret0.8/4 & human & 76.6 & 2000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RPN-Rerank & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $44.7\pm 20.9$ &  & $1626.6\pm 178.8$ &  & human & 77.4 & 3000\\
 &  &  &  & ret0.6/1 & human & 77.1 & 3000\\
$11.8\pm 2.2$ & $41.7\pm 17.0$ & $26.8\pm 15.6$ & $1633.1\pm 183.3$ & ret0.7/1 & human & 77.3 & 3000\\
 &  &  &  & ret0.73/1 & human & 77.1 & 3000\\
$12.6\pm 2.2$ & $52.3\pm 20.2$ & $37.1\pm 19.1$ & $1560.7\pm 189.8$ & ret0.8/1 & human & 77.4 & 3000\\
 &  &  &  & ret0.6/2 & human & 76.8 & 3000\\
$16.8\pm 3.4$ & $36.7\pm 11.7$ & $17.6\pm 9.3$ & $1616.4\pm 178.5$ & ret0.7/2 & human & 77.2 & 3000\\
 &  &  &  & ret0.73/2 & human & 77.0 & 3000\\
$22.3\pm 4.2$ & $57.1\pm 17.9$ & $32.2\pm 15.6$ & $1519.7\pm 197.4$ & ret0.8/2 & human & 77.3 & 3000\\
 &  &  &  & ret0.6/3 & human & 76.5 & 3000\\
$21.6\pm 4.2$ & $39.9\pm 13.7$ & $15.8\pm 10.3$ & $1656.4\pm 183.3$ & ret0.7/3 & human & 77.0 & 3000\\
 &  &  &  & ret0.73/3 & human & 77.0 & 3000\\
$29.3\pm 6.0$ & $61.9\pm 21.9$ & $30.3\pm 17.5$ & $1670.1\pm 178.4$ & ret0.8/3 & human & 77.3 & 3000\\
 &  &  &  & ret0.6/4 & human & 76.3 & 3000\\
$26.1\pm 6.3$ & $42.7\pm 14.6$ & $14.2\pm 9.0$ & $1550.7\pm 195.0$ & ret0.7/4 & human & 77.0 & 3000\\
 &  &  &  & ret0.73/4 & human & 76.9 & 3000\\
$37.2\pm 7.4$ & $69.9\pm 21.5$ & $30.1\pm 16.1$ & $1547.8\pm 177.0$ & ret0.8/4 & human & 77.3 & 3000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RPN-Rerank & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $163.5\pm 64.1$ &  & $1736.0\pm 194.6$ &  & human & 77.9 & 6000\\
 &  &  &  & ret0.6/1 & human & 77.6 & 6000\\
$21.1\pm 3.0$ & $141.9\pm 56.6$ & $116.3\pm 55.1$ & $1788.5\pm 291.2$ & ret0.7/1 & human & 77.7 & 6000\\
 &  &  &  & ret0.73/1 & human & 77.6 & 6000\\
$21.7\pm 3.9$ & $181.9\pm 71.4$ & $156.2\pm 69.4$ & $1696.9\pm 223.9$ & ret0.8/1 & human & 77.8 & 6000\\
 &  &  &  & ret0.6/2 & human & 77.3 & 6000\\
$30.5\pm 5.4$ & $116.3\pm 44.9$ & $82.2\pm 41.2$ & $1705.5\pm 199.7$ & ret0.7/2 & human & 0.0 & 6000\\
 &  &  &  & ret0.73/2 & human & 77.5 & 6000\\
$39.4\pm 7.1$ & $188.9\pm 70.8$ & $145.7\pm 67.0$ & $1721.0\pm 240.9$ & ret0.8/2 & human & 77.8 & 6000\\
 &  &  &  & ret0.6/3 & human & 77.0 & 6000\\
$40.0\pm 7.7$ & $114.3\pm 44.3$ & $70.5\pm 38.9$ & $1704.5\pm 185.9$ & ret0.7/3 & human & 77.5 & 6000\\
 &  &  &  & ret0.73/3 & human & 77.4 & 6000\\
$55.1\pm 10.0$ & $199.3\pm 69.3$ & $140.4\pm 63.0$ & $1778.9\pm 204.7$ & ret0.8/3 & human & 77.8 & 6000\\
 &  &  &  & ret0.6/4 & human & 76.8 & 6000\\
$49.8\pm 9.3$ & $118.1\pm 42.3$ & $64.1\pm 35.2$ & $1749.3\pm 197.9$ & ret0.7/4 & human & 77.5 & 6000\\
 &  &  &  & ret0.73/4 & human & 77.3 & 6000\\
$67.0\pm 10.8$ & $202.4\pm 64.6$ & $131.5\pm 58.8$ & $1716.1\pm 184.6$ & ret0.8/4 & human & 77.7 & 6000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RPN-Rerank & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $327.8\pm 104.8$ &  & $1870.9\pm 201.3$ &  & human & 77.7 & 9000\\
 &  &  &  & ret0.6/1 & human & 77.7 & 9000\\
$27.5\pm 4.0$ & $270.1\pm 92.4$ & $237.1\pm 90.7$ & $1832.3\pm 215.6$ & ret0.7/1 & human & 77.8 & 9000\\
$22.2\pm 2.8$ & $282.7\pm 98.5$ & $256.3\pm 96.9$ & $1672.6\pm 223.2$ & ret0.73/1 & human & 77.9 & 9000\\
$29.0\pm 5.2$ & $333.2\pm 117.6$ & $298.8\pm 114.6$ & $1919.2\pm 219.8$ & ret0.75/1 & human & 77.7 & 9000\\
$32.1\pm 5.5$ & $374.8\pm 121.5$ & $337.0\pm 119.4$ & $1985.1\pm 233.5$ & ret0.8/1 & human & 77.9 & 9000\\
 &  &  &  & ret0.6/2 & human & 77.4 & 9000\\
$44.1\pm 7.4$ & $243.4\pm 87.1$ & $194.1\pm 82.4$ & $1853.5\pm 209.1$ & ret0.7/2 & human & 77.7 & 9000\\
$42.2\pm 6.5$ & $281.6\pm 91.4$ & $234.5\pm 88.7$ & $1837.4\pm 212.5$ & ret0.73/2 & human & 77.6 & 9000\\
 &  &  &  & ret0.75/2 & human & 77.6 & 9000\\
$53.6\pm 8.4$ & $376.5\pm 118.3$ & $317.8\pm 114.8$ & $1907.1\pm 250.8$ & ret0.8/2 & human & 77.9 & 9000\\
 &  &  &  & ret0.6/3 & human & 77.1 & 9000\\
$56.5\pm 10.0$ & $230.3\pm 79.5$ & $168.8\pm 73.4$ & $1779.8\pm 197.2$ & ret0.7/3 & human & 77.6 & 9000\\
$56.8\pm 9.0$ & $278.5\pm 93.7$ & $216.4\pm 87.3$ & $1858.9\pm 209.7$ & ret0.73/3 & human & 77.5 & 9000\\
 &  &  &  & ret0.75/3 & human & 77.6 & 9000\\
$76.1\pm 12.7$ & $390.0\pm 122.4$ & $308.4\pm 115.6$ & $1936.5\pm 252.9$ & ret0.8/3 & human & 77.9 & 9000\\
 &  &  &  & ret0.6/4 & human & 76.9 & 9000\\
$68.6\pm 11.5$ & $227.0\pm 78.2$ & $153.4\pm 70.3$ & $1834.9\pm 222.4$ & ret0.7/4 & human & 77.6 & 9000\\
$66.2\pm 10.6$ & $264.5\pm 93.3$ & $193.5\pm 85.2$ & $1841.9\pm 210.1$ & ret0.73/4 & human & 77.4 & 9000\\
 &  &  &  & ret0.75/4 & human & 77.5 & 9000\\
$92.0\pm 15.2$ & $387.4\pm 120.8$ & $290.3\pm 111.0$ & $1994.2\pm 250.1$ & ret0.8/4 & human & 77.8 & 9000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RPN-Rerank & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $371.0\pm 118.1$ &  & $1882.9\pm 213.2$ &  & human & 77.8 & 10000\\
$27.9\pm 3.9$ & $308.7\pm 102.8$ & $275.3\pm 101.4$ & $1896.4\pm 221.7$ & ret0.7/1 & human & 77.6 & 10000\\
$30.6\pm 4.8$ & $355.0\pm 121.2$ & $318.6\pm 118.9$ & $1936.7\pm 231.4$ & ret0.73/1 & human & 77.7 & 10000\\
$32.8\pm 5.9$ & $390.7\pm 132.5$ & $351.8\pm 130.7$ & $1979.6\pm 233.1$ & ret0.75/1 & human & 77.7 & 10000\\
$34.0\pm 5.2$ & $438.4\pm 141.6$ & $398.2\pm 139.4$ & $2056.3\pm 244.6$ & ret0.8/1 & human & 77.7 & 10000\\
 &  &  &  & ret0.7/2 & human & 77.5 & 10000\\
 &  &  &  & ret0.73/2 & human & 77.6 & 10000\\
 &  &  &  & ret0.75/2 & human & 77.6 & 10000\\
 &  &  &  & ret0.8/2 & human & 77.7 & 10000\\
 &  &  &  & ret0.7/3 & human & 77.4 & 10000\\
 &  &  &  & ret0.73/3 & human & 77.5 & 10000\\
 &  &  &  & ret0.75/3 & human & 77.6 & 10000\\
 &  &  &  & ret0.8/3 & human & 77.7 & 10000\\
 &  &  &  & ret0.7/4 & human & 77.4 & 10000\\
 &  &  &  & ret0.73/4 & human & 77.4 & 10000\\
 &  &  &  & ret0.75/4 & human & 77.5 & 10000\\
 &  &  &  & ret0.8/4 & human & 77.6 & 10000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RPN-Rerank & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $538.3\pm 175.1$ &  & $2115.1\pm 267.7$ &  & human & 78.0 & 12000\\
 &  &  &  & ret0.6/1 & human & 77.7 & 12000\\
$33.0\pm 4.9$ & $413.2\pm 139.2$ & $373.8\pm 137.6$ & $2010.1\pm 244.6$ & ret0.7/1 & human & 77.9 & 12000\\
 &  &  &  & ret0.73/1 & human & 77.7 & 12000\\
$36.4\pm 5.5$ & $564.3\pm 175.6$ & $521.6\pm 175.4$ & $2076.0\pm 260.8$ & ret0.8/1 & human & 77.9 & 12000\\
 &  &  &  & ret0.6/2 & human & 77.4 & 12000\\
$52.9\pm 9.3$ & $366.1\pm 128.6$ & $307.6\pm 123.5$ & $1970.2\pm 240.7$ & ret0.7/2 & human & 77.7 & 12000\\
 &  &  &  & ret0.73/2 & human & 77.6 & 12000\\
$65.6\pm 10.9$ & $566.5\pm 181.8$ & $495.1\pm 177.5$ & $2106.0\pm 266.1$ & ret0.8/2 & human & 77.9 & 12000\\
 &  &  &  & ret0.6/3 & human & 77.2 & 12000\\
$69.1\pm 11.8$ & $342.6\pm 108.9$ & $267.8\pm 102.4$ & $1946.3\pm 222.0$ & ret0.7/3 & human & 77.7 & 12000\\
 &  &  &  & ret0.73/3 & human & 77.5 & 12000\\
$88.5\pm 15.0$ & $572.2\pm 182.8$ & $478.1\pm 177.6$ & $2174.1\pm 286.8$ & ret0.8/3 & human & 77.9 & 12000\\
 &  &  &  & ret0.6/4 & human & 76.9 & 12000\\
$83.2\pm 16.1$ & $326.9\pm 109.0$ & $238.2\pm 96.9$ & $1877.8\pm 233.0$ & ret0.7/4 & human & 77.6 & 12000\\
 &  &  &  & ret0.73/4 & human & 77.5 & 12000\\
$111.7\pm 18.7$ & $578.3\pm 180.6$ & $460.9\pm 170.1$ & $2112.0\pm 258.2$ & ret0.8/4 & human & 77.8 & 12000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RPN-Rerank & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $21.0\pm 4.2$ &  & $1700.0\pm 711.5$ &  & sku & 83.4 & 2000\\
 &  &  &  & ret0.6/1 & sku & 83.4 & 2000\\
$7.8\pm 1.5$ & $21.5\pm 4.7$ & $11.4\pm 3.1$ & $1529.3\pm 172.8$ & ret0.7/1 & sku & 83.4 & 2000\\
 &  &  &  & ret0.73/1 & sku & 83.4 & 2000\\
$8.4\pm 1.4$ & $26.8\pm 5.5$ & $16.1\pm 4.3$ & $1463.0\pm 146.0$ & ret0.8/1 & sku & 83.4 & 2000\\
 &  &  &  & ret0.6/2 & sku & 83.3 & 2000\\
$10.4\pm 1.9$ & $19.8\pm 3.9$ & $7.7\pm 2.0$ & $1414.1\pm 201.1$ & ret0.7/2 & sku & 83.4 & 2000\\
 &  &  &  & ret0.73/2 & sku & 83.4 & 2000\\
$13.9\pm 2.8$ & $29.6\pm 6.6$ & $13.7\pm 3.7$ & $1502.4\pm 170.4$ & ret0.8/2 & sku & 83.4 & 2000\\
 &  &  &  & ret0.6/3 & sku & 83.3 & 2000\\
$14.0\pm 2.6$ & $22.6\pm 4.8$ & $6.9\pm 2.1$ & $1505.2\pm 184.8$ & ret0.7/3 & sku & 83.4 & 2000\\
 &  &  &  & ret0.73/3 & sku & 83.4 & 2000\\
$18.0\pm 3.9$ & $32.6\pm 8.0$ & $12.7\pm 4.0$ & $1474.4\pm 176.5$ & ret0.8/3 & sku & 83.4 & 2000\\
 &  &  &  & ret0.6/4 & sku & 83.3 & 2000\\
$16.8\pm 3.4$ & $25.0\pm 5.4$ & $6.5\pm 1.9$ & $1502.3\pm 176.1$ & ret0.7/4 & sku & 83.4 & 2000\\
 &  &  &  & ret0.73/4 & sku & 83.4 & 2000\\
$22.3\pm 4.3$ & $36.2\pm 7.2$ & $12.1\pm 3.3$ & $1529.3\pm 179.8$ & ret0.8/4 & sku & 83.4 & 2000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RPN-Rerank & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $33.0\pm 8.8$ &  & $1468.1\pm 243.8$ &  & sku & 87.3 & 3000\\
 &  &  &  & ret0.6/1 & sku & 87.2 & 3000\\
$10.5\pm 2.0$ & $32.3\pm 7.4$ & $18.9\pm 5.5$ & $1496.0\pm 153.4$ & ret0.7/1 & sku & 87.2 & 3000\\
 &  &  &  & ret0.73/1 & sku & 87.2 & 3000\\
$11.9\pm 2.5$ & $39.6\pm 9.0$ & $24.9\pm 6.8$ & $1439.5\pm 175.1$ & ret0.8/1 & sku & 87.3 & 3000\\
 &  &  &  & ret0.6/2 & sku & 87.1 & 3000\\
$14.1\pm 2.6$ & $29.4\pm 6.1$ & $13.0\pm 3.7$ & $1511.4\pm 192.4$ & ret0.7/2 & sku & 87.2 & 3000\\
 &  &  &  & ret0.73/2 & sku & 87.2 & 3000\\
$18.2\pm 3.5$ & $42.7\pm 10.6$ & $22.2\pm 7.2$ & $1539.6\pm 161.7$ & ret0.8/2 & sku & 87.2 & 3000\\
 &  &  &  & ret0.6/3 & sku & 87.1 & 3000\\
$17.9\pm 3.4$ & $30.6\pm 6.1$ & $10.6\pm 2.9$ & $1533.7\pm 185.0$ & ret0.7/3 & sku & 87.2 & 3000\\
 &  &  &  & ret0.73/3 & sku & 87.2 & 3000\\
$23.4\pm 4.8$ & $46.3\pm 11.6$ & $20.6\pm 7.0$ & $1496.9\pm 192.0$ & ret0.8/3 & sku & 87.2 & 3000\\
 &  &  &  & ret0.6/4 & sku & 87.1 & 3000\\
$22.2\pm 4.5$ & $34.6\pm 7.3$ & $10.1\pm 2.8$ & $1505.0\pm 183.1$ & ret0.7/4 & sku & 87.2 & 3000\\
 &  &  &  & ret0.73/4 & sku & 87.2 & 3000\\
$28.7\pm 5.7$ & $50.3\pm 10.6$ & $19.4\pm 5.4$ & $1507.2\pm 167.3$ & ret0.8/4 & sku & 87.2 & 3000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RPN-Rerank & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $93.4\pm 28.5$ &  & $1658.3\pm 812.4$ &  & sku & 90.8 & 6000\\
 &  &  &  & ret0.6/1 & sku & 90.6 & 6000\\
$17.9\pm 2.8$ & $76.1\pm 21.0$ & $53.9\pm 18.8$ & $1553.9\pm 194.5$ & ret0.7/1 & sku & 90.7 & 6000\\
 &  &  &  & ret0.73/1 & sku & 90.7 & 6000\\
$19.7\pm 3.4$ & $102.6\pm 27.2$ & $78.9\pm 24.8$ & $1571.4\pm 188.5$ & ret0.8/1 & sku & 90.7 & 6000\\
 &  &  &  & ret0.6/2 & sku & 90.5 & 6000\\
$24.8\pm 4.5$ & $67.9\pm 16.7$ & $39.3\pm 12.8$ & $1500.1\pm 188.2$ & ret0.7/2 & sku & 90.6 & 6000\\
 &  &  &  & ret0.73/2 & sku & 90.7 & 6000\\
$31.8\pm 5.2$ & $108.0\pm 27.4$ & $72.6\pm 23.5$ & $1501.5\pm 173.6$ & ret0.8/2 & sku & 90.7 & 6000\\
 &  &  &  & ret0.6/3 & sku & 90.5 & 6000\\
$32.7\pm 5.6$ & $70.3\pm 15.6$ & $33.8\pm 10.5$ & $1520.3\pm 197.6$ & ret0.7/3 & sku & 90.6 & 6000\\
 &  &  &  & ret0.73/3 & sku & 90.6 & 6000\\
$43.7\pm 7.5$ & $116.1\pm 29.3$ & $68.7\pm 23.9$ & $1586.9\pm 185.1$ & ret0.8/3 & sku & 90.7 & 6000\\
 &  &  &  & ret0.6/4 & sku & 90.4 & 6000\\
$36.3\pm 6.9$ & $68.3\pm 16.3$ & $28.5\pm 9.7$ & $1503.6\pm 171.1$ & ret0.7/4 & sku & 90.6 & 6000\\
 &  &  &  & ret0.73/4 & sku & 90.6 & 6000\\
$49.7\pm 8.4$ & $116.1\pm 28.2$ & $63.0\pm 20.9$ & $1562.3\pm 190.5$ & ret0.8/4 & sku & 90.7 & 6000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RPN-Rerank & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $185.2\pm 41.7$ &  & $1640.9\pm 172.5$ &  & sku & 91.6 & 9000\\
$20.9\pm 4.3$ & $77.6\pm 21.3$ & $51.2\pm 17.8$ & $1503.1\pm 196.8$ & ret0.6/1 & sku & 91.5 & 9000\\
$25.5\pm 4.5$ & $147.4\pm 41.9$ & $116.0\pm 38.6$ & $1606.8\pm 172.5$ & ret0.7/1 & sku & 91.5 & 9000\\
$19.4\pm 3.5$ & $148.4\pm 41.2$ & $124.5\pm 38.5$ & $1576.3\pm 222.5$ & ret0.73/1 & sku & 91.6 & 9000\\
$24.3\pm 3.7$ & $166.1\pm 42.6$ & $136.8\pm 40.4$ & $1631.5\pm 193.4$ & ret0.75/1 & sku & 91.6 & 9000\\
$26.4\pm 4.3$ & $192.8\pm 49.5$ & $161.2\pm 46.5$ & $1646.6\pm 218.3$ & ret0.8/1 & sku & 91.6 & 9000\\
 &  &  &  & ret0.6/2 & sku & 91.4 & 9000\\
$35.3\pm 6.1$ & $122.0\pm 33.0$ & $81.9\pm 28.4$ & $1617.1\pm 170.3$ & ret0.7/2 & sku & 91.5 & 9000\\
$33.9\pm 5.8$ & $142.6\pm 39.9$ & $104.2\pm 35.6$ & $1567.6\pm 194.3$ & ret0.73/2 & sku & 91.6 & 9000\\
 &  &  &  & ret0.75/2 & sku & 91.5 & 9000\\
$44.4\pm 7.1$ & $201.1\pm 49.6$ & $151.6\pm 44.2$ & $1679.5\pm 186.5$ & ret0.8/2 & sku & 91.6 & 9000\\
 &  &  &  & ret0.6/3 & sku & 91.3 & 9000\\
$45.0\pm 7.2$ & $118.9\pm 28.0$ & $68.7\pm 22.0$ & $1599.4\pm 180.1$ & ret0.7/3 & sku & 91.4 & 9000\\
$42.7\pm 6.8$ & $135.4\pm 34.5$ & $88.2\pm 29.1$ & $1571.8\pm 173.1$ & ret0.73/3 & sku & 91.5 & 9000\\
 &  &  &  & ret0.75/3 & sku & 91.5 & 9000\\
$56.0\pm 8.5$ & $198.8\pm 48.5$ & $138.2\pm 41.7$ & $1668.5\pm 190.1$ & ret0.8/3 & sku & 91.6 & 9000\\
 &  &  &  & ret0.6/4 & sku & 91.2 & 9000\\
$55.2\pm 8.9$ & $124.3\pm 28.9$ & $63.6\pm 21.4$ & $1625.1\pm 176.1$ & ret0.7/4 & sku & 91.4 & 9000\\
$50.3\pm 8.2$ & $135.9\pm 34.5$ & $81.0\pm 27.5$ & $1531.5\pm 210.9$ & ret0.73/4 & sku & 91.5 & 9000\\
 &  &  &  & ret0.75/4 & sku & 91.5 & 9000\\
$73.9\pm 12.7$ & $218.8\pm 55.1$ & $139.8\pm 45.5$ & $1707.0\pm 191.2$ & ret0.8/4 & sku & 91.5 & 9000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RPN-Rerank & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $197.8\pm 47.4$ &  & $1629.4\pm 188.0$ &  & sku & 91.8 & 10000\\
$25.0\pm 4.2$ & $155.4\pm 46.2$ & $124.9\pm 42.8$ & $1627.4\pm 172.5$ & ret0.7/1 & sku & 91.7 & 10000\\
$27.5\pm 4.2$ & $188.1\pm 48.3$ & $154.6\pm 45.6$ & $1582.9\pm 211.5$ & ret0.73/1 & sku & 91.8 & 10000\\
$26.1\pm 4.1$ & $191.4\pm 49.8$ & $159.9\pm 47.2$ & $1621.5\pm 209.6$ & ret0.75/1 & sku & 91.8 & 10000\\
$29.7\pm 4.6$ & $231.3\pm 54.5$ & $195.6\pm 51.5$ & $1675.7\pm 207.3$ & ret0.8/1 & sku & 91.8 & 10000\\
 &  &  &  & ret0.7/2 & sku & 91.6 & 10000\\
 &  &  &  & ret0.73/2 & sku & 91.7 & 10000\\
 &  &  &  & ret0.75/2 & sku & 91.8 & 10000\\
 &  &  &  & ret0.8/2 & sku & 91.8 & 10000\\
 &  &  &  & ret0.7/3 & sku & 91.6 & 10000\\
 &  &  &  & ret0.73/3 & sku & 91.7 & 10000\\
 &  &  &  & ret0.75/3 & sku & 91.6 & 10000\\
 &  &  &  & ret0.8/3 & sku & 91.7 & 10000\\
 &  &  &  & ret0.7/4 & sku & 91.5 & 10000\\
 &  &  &  & ret0.73/4 & sku & 91.6 & 10000\\
 &  &  &  & ret0.75/4 & sku & 91.6 & 10000\\
 &  &  &  & ret0.8/4 & sku & 91.7 & 10000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RPN-Rerank & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $281.3\pm 60.9$ &  & $1746.9\pm 165.6$ &  & sku & 91.9 & 12000\\
 &  &  &  & ret0.6/1 & sku & 91.8 & 12000\\
$32.6\pm 2.8$ & $237.5\pm 52.4$ & $197.1\pm 50.5$ & $1706.5\pm 198.6$ & ret0.7/1 & sku & 91.8 & 12000\\
 &  &  &  & ret0.73/1 & sku & 91.8 & 12000\\
$33.2\pm 5.6$ & $287.2\pm 68.2$ & $247.8\pm 64.5$ & $1775.4\pm 222.4$ & ret0.8/1 & sku & 91.9 & 12000\\
 &  &  &  & ret0.6/2 & sku & 91.6 & 12000\\
$44.1\pm 7.8$ & $183.4\pm 50.4$ & $133.7\pm 44.3$ & $1647.6\pm 180.4$ & ret0.7/2 & sku & 91.8 & 12000\\
 &  &  &  & ret0.73/2 & sku & 91.8 & 12000\\
$52.2\pm 7.3$ & $281.2\pm 61.4$ & $223.5\pm 56.6$ & $1664.5\pm 174.3$ & ret0.8/2 & sku & 91.9 & 12000\\
 &  &  &  & ret0.6/3 & sku & 91.6 & 12000\\
$54.1\pm 8.2$ & $169.5\pm 40.6$ & $109.9\pm 33.9$ & $1636.7\pm 191.8$ & ret0.7/3 & sku & 91.7 & 12000\\
 &  &  &  & ret0.73/3 & sku & 91.8 & 12000\\
$72.0\pm 11.6$ & $296.0\pm 66.9$ & $218.1\pm 58.3$ & $1734.8\pm 204.3$ & ret0.8/3 & sku & 91.9 & 12000\\
 &  &  &  & ret0.6/4 & sku & 91.5 & 12000\\
$63.5\pm 11.1$ & $165.5\pm 42.0$ & $96.2\pm 32.7$ & $1656.5\pm 172.8$ & ret0.7/4 & sku & 91.7 & 12000\\
 &  &  &  & ret0.73/4 & sku & 91.8 & 12000\\
$85.3\pm 13.9$ & $295.8\pm 63.2$ & $204.9\pm 54.0$ & $1747.2\pm 201.2$ & ret0.8/4 & sku & 91.8 & 12000\\
\bottomrule
\end{tabular}
\end{table*}

==> table/retina_table.tex <==
\begin{table}
\centering
\caption{Experiment results on CARPK with Retina-R50-FPN. The columns of HNMS, NMS and Total represent the time cost in ms. Speed is for the total cost by HNMS and NMS.}
\label{tbl:retina_CARPK}
\begin{tabular}{c@{~}c@{~}c@{~~}c@{~~}c@{~~}c@{~~}c}
\toprule
 & $K$ & mAP & HNMS & NMS & Speed & Total\\
\midrule
NMS &  & 94.8 &  & $260.9\pm 104.8$ & 1x & $2071.1\pm 230.5$\\
\midrule
\multirow{4}{*}{HNMS} & 1 & \textbf{95.3} & $23.6\pm 4.9$ & $194.2\pm 100.9$ & \textbf{1.20x} & $1761.9\pm 149.7$\\
 & 2 & \textbf{95.3} & $34.0\pm 6.4$ & $161.7\pm 88.6$ & \textbf{1.33x} & $1762.6\pm 187.2$\\
 & 3 & 95.2 & $46.1\pm 8.5$ & $140.4\pm 80.2$ & 1.40x & $1794.6\pm 108.5$\\
 & 4 & 95.2 & $51.4\pm 8.4$ & $122.4\pm 67.8$ & 1.50x & $1732.6\pm 129.7$\\
\bottomrule
\end{tabular}
\end{table}\begin{table}
\centering
\caption{Experiment results on SKU-110K with Retina-R50-FPN. The columns of HNMS, NMS and Total represent the time cost in ms. Speed is for the total cost by HNMS and NMS.}
\label{tbl:retina_SKU-110K}
\begin{tabular}{c@{~}c@{~}c@{~~}c@{~~}c@{~~}c@{~~}c}
\toprule
 & $K$ & mAP & HNMS & NMS & Speed & Total\\
\midrule
NMS &  & \textbf{91.6} &  & $185.2\pm 41.7$ & \textbf{1x} & $1640.9\pm 172.5$\\
\midrule
\multirow{4}{*}{HNMS} & 1 & \textbf{91.6} & $19.4\pm 3.5$ & $124.5\pm 38.5$ & \textbf{1.29x} & $1576.3\pm 222.5$\\
 & 2 & \textbf{91.6} & $33.9\pm 5.8$ & $104.2\pm 35.6$ & \textbf{1.34x} & $1567.6\pm 194.3$\\
 & 3 & 91.5 & $42.7\pm 6.8$ & $88.2\pm 29.1$ & 1.41x & $1571.8\pm 173.1$\\
 & 4 & 91.5 & $50.3\pm 8.2$ & $81.0\pm 27.5$ & 1.41x & $1531.5\pm 210.9$\\
\bottomrule
\end{tabular}
\end{table}\begin{table}
\centering
\caption{Experiment results on CrowdHuman with Retina-R50-FPN. The columns of HNMS, NMS and Total represent the time cost in ms. Speed is for the total cost by HNMS and NMS.}
\label{tbl:retina_CrowdHuman}
\begin{tabular}{c@{~}c@{~}c@{~~}c@{~~}c@{~~}c@{~~}c}
\toprule
 & $K$ & mAP & HNMS & NMS & Speed & Total\\
\midrule
NMS &  & 77.7 &  & $327.8\pm 104.8$ & 1x & $1870.9\pm 201.3$\\
\midrule
\multirow{4}{*}{HNMS} & 1 & \textbf{77.8} & $25.0\pm 4.2$ & $268.7\pm 107.0$ & \textbf{1.12x} & $1653.4\pm 233.2$\\
 & 2 & 77.6 & $42.2\pm 6.5$ & $234.5\pm 88.7$ & 1.18x & $1837.4\pm 212.5$\\
 & 3 & 77.5 & $56.8\pm 9.0$ & $216.4\pm 87.3$ & 1.20x & $1858.9\pm 209.7$\\
 & 4 & 77.4 & $66.2\pm 10.6$ & $193.5\pm 85.2$ & 1.26x & $1841.9\pm 210.1$\\
\bottomrule
\end{tabular}
\end{table}

==> table/retina_table1.bak.tex <==
\begin{table}
\centering

\caption{Experiment results with Retina-R50-FPN.
	The columns of HNMS, NMS and Total represent the time cost in ms.
	Speed is for the total cost relative to NMS.}

\label{tbl:retina}
\begin{tabular}{c}
(a) CARPK
\\	
\begin{tabular}{c@{~}c@{~}c@{~~}c@{~~}c@{~~}c}
\toprule
 & $K$ & mAP & HNMS & NMS & Speed\\
\midrule
NMS &  & 94.8 &  & $260.9\pm 104.8$ & 1x\\
\midrule
\multirow{4}{*}{HNMS} & 1 & \textbf{95.3} & $23.6\pm 4.9$ & $194.2\pm 100.9$ & \textbf{1.20x}\\
 & 2 & \textbf{95.3} & $34.0\pm 6.4$ & $161.7\pm 88.6$ & \textbf{1.33x}\\
 & 3 & 95.2 & $46.1\pm 8.5$ & $140.4\pm 80.2$ & 1.40x\\
 & 4 & 95.2 & $51.4\pm 8.4$ & $122.4\pm 67.8$ & 1.50x\\
\bottomrule
\end{tabular}
\\
\\
(b) SKU-110K
\\
\begin{tabular}{c@{~}c@{~}c@{~~}c@{~~}c@{~~}c}
\toprule
 & $K$ & mAP & HNMS & NMS & Speed\\
\midrule
NMS &  & \textbf{91.6} &  & $185.2\pm 41.7$ & \textbf{1x}\\
\midrule
\multirow{4}{*}{HNMS} & 1 & \textbf{91.6} & $19.4\pm 3.5$ & $124.5\pm 38.5$ & \textbf{1.29x}\\
 & 2 & \textbf{91.6} & $33.9\pm 5.8$ & $104.2\pm 35.6$ & \textbf{1.34x}\\
 & 3 & 91.5 & $42.7\pm 6.8$ & $88.2\pm 29.1$ & 1.41x\\
 & 4 & 91.5 & $50.3\pm 8.2$ & $81.0\pm 27.5$ & 1.41x\\
\bottomrule
\end{tabular}
\\
\\
(c) CrowdHuman
\\
\begin{tabular}{c@{~}c@{~}c@{~~}c@{~~}c@{~~}c}
\toprule
 & $K$ & mAP & HNMS & NMS & Speed\\
\midrule
NMS &  & 77.7 &  & $327.8\pm 104.8$ & 1x\\
\midrule
\multirow{4}{*}{HNMS} & 1 & \textbf{77.9} & $22.2\pm 2.8$ & $256.3\pm 96.9$ & \textbf{1.18x}\\
 & 2 & 77.6 & $42.2\pm 6.5$ & $234.5\pm 88.7$ & 1.18x\\
 & 3 & 77.5 & $56.8\pm 9.0$ & $216.4\pm 87.3$ & 1.20x\\
 & 4 & 77.4 & $66.2\pm 10.6$ & $193.5\pm 85.2$ & 1.26x\\
\bottomrule
\end{tabular}
\end{tabular}

\end{table}

==> table/retina_table1.tex <==
\begin{table}
\centering

\caption{Experiment results with Retina-R50-FPN.
	The columns of HNMS, NMS and Total represent the time cost in ms.
	Speed is for the total cost consumed by HNMS and NMS. HNMS is as a pre-filter
	to reduce the total time cost.}

\label{tbl:retina}
\begin{tabular}{c}
(a) CARPK
\\	
\begin{tabular}{c@{~}c@{~}c@{~~}c@{~~}c@{~~}c}
\toprule
 & $K$ & mAP & HNMS & NMS & Speed\\
\midrule
NMS &  & 94.8 &  & $260.9\pm 104.8$ & 1x\\
\midrule
 & 1 & \textbf{95.3} & $23.6\pm 4.9$ & $194.2\pm 100.9$ & \textbf{1.20x}\\
 HNMS & 2 & \textbf{95.3} & $34.0\pm 6.4$ & $161.7\pm 88.6$ & \textbf{1.33x}\\
 +NMS & 3 & 95.2 & $46.1\pm 8.5$ & $140.4\pm 80.2$ & 1.40x\\
 & 4 & 95.2 & $51.4\pm 8.4$ & $122.4\pm 67.8$ & 1.50x\\
\bottomrule
\end{tabular}
\\
\\
(b) SKU-110K
\\
\begin{tabular}{c@{~}c@{~}c@{~~}c@{~~}c@{~~}c}
\toprule
 & $K$ & mAP & HNMS & NMS & Speed\\
\midrule
NMS &  & \textbf{91.6} &  & $185.2\pm 41.7$ & \textbf{1x}\\
\midrule
 & 1 & \textbf{91.6} & $19.4\pm 3.5$ & $124.5\pm 38.5$ & \textbf{1.29x}\\
 HNMS & 2 & \textbf{91.6} & $33.9\pm 5.8$ & $104.2\pm 35.6$ & \textbf{1.34x}\\
 +NMS & 3 & 91.5 & $42.7\pm 6.8$ & $88.2\pm 29.1$ & 1.41x\\
 & 4 & 91.5 & $50.3\pm 8.2$ & $81.0\pm 27.5$ & 1.41x\\
\bottomrule
\end{tabular}
%\\
%\\
%(c) CrowdHuman
%\\
%\begin{tabular}{c@{~}c@{~}c@{~~}c@{~~}c@{~~}c}
%	\toprule
%	& $K$ & mAP & HNMS & NMS & Speed\\
%	\midrule
%	NMS &  & 77.7 &  & $327.8\pm 104.8$ & 1x\\
%	\midrule
%	& 1 & \textbf{77.8} & $22.2\pm 2.8$ & $256.3\pm 96.9$ & \textbf{1.18x}\\
%	HNMS & 2 & 77.6 & $42.2\pm 6.5$ & $234.5\pm 88.7$ & 1.18x\\
%	+NMS & 3 & 77.5 & $56.8\pm 9.0$ & $216.4\pm 87.3$ & 1.20x\\
%	& 4 & 77.4 & $66.2\pm 10.6$ & $193.5\pm 85.2$ & 1.26x\\
%	\bottomrule
%\end{tabular}
\end{tabular}

\end{table}

==> table/rpn.tex <==
\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RoI-NMS & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $5.4\pm 0.9$ & $1.1\pm 0.4$ & $2384.3\pm 167.1$ &  & car & 95.0 & 1000\\
$4.4\pm 0.8$ & $6.7\pm 1.4$ & $1.9\pm 0.6$ & $2904.5\pm 151.0$ & rpn0.7/1 & car & 95.1 & 1000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RoI-NMS & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $33.0\pm 5.8$ & $2.8\pm 1.2$ & $3245.5\pm 210.3$ &  & car & 96.3 & 3000\\
$9.5\pm 1.8$ & $13.0\pm 2.5$ & $3.5\pm 1.3$ & $3518.7\pm 231.4$ & rpn0.7/1 & car & 96.4 & 3000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RoI-NMS & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $103.5\pm 16.9$ & $3.6\pm 1.4$ & $3789.7\pm 177.6$ &  & car & 96.7 & 6000\\
$15.5\pm 2.5$ & $21.0\pm 3.6$ & $3.0\pm 1.1$ & $3664.7\pm 193.4$ & rpn0.7/1 & car & 97.0 & 6000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RoI-NMS & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $223.3\pm 36.5$ & $3.3\pm 1.3$ & $3935.7\pm 184.9$ &  & car & 96.9 & 9000\\
 &  &  &  & rpn0.4/2 & car & 96.2 & 9000\\
 &  &  &  & rpn0.4/3 & car & 96.1 & 9000\\
 &  &  &  & rpn0.4/4 & car & 96.0 & 9000\\
 &  &  &  & rpn0.5/1 & car & 96.1 & 9000\\
 &  &  &  & rpn0.5/2 & car & 96.1 & 9000\\
 &  &  &  & rpn0.5/3 & car & 96.1 & 9000\\
 &  &  &  & rpn0.5/4 & car & 96.2 & 9000\\
 &  &  &  & rpn0.6/1 & car & 96.5 & 9000\\
 &  &  &  & rpn0.6/2 & car & 96.1 & 9000\\
 &  &  &  & rpn0.6/3 & car & 96.1 & 9000\\
$37.0\pm 5.6$ & $42.9\pm 6.8$ & $1.8\pm 0.8$ & $3114.1\pm 219.8$ & rpn0.6/4 & car & 96.1 & 9000\\
$22.6\pm 3.8$ & $30.3\pm 5.4$ & $2.9\pm 1.0$ & $3665.6\pm 205.4$ & rpn0.7/1 & car & 97.1 & 9000\\
$41.0\pm 5.0$ & $49.0\pm 6.5$ & $3.2\pm 1.3$ & $3571.5\pm 172.0$ & rpn0.7/2 & car & 97.1 & 9000\\
$44.6\pm 6.3$ & $52.3\pm 7.6$ & $3.4\pm 1.3$ & $3790.5\pm 186.1$ & rpn0.7/3 & car & 97.0 & 9000\\
$60.9\pm 8.1$ & $68.8\pm 9.6$ & $3.4\pm 1.3$ & $3790.6\pm 467.3$ & rpn0.7/4 & car & 96.9 & 9000\\
 &  &  &  & rpn0.8/1 & car & 96.2 & 9000\\
 &  &  &  & rpn0.8/2 & car & 96.3 & 9000\\
 &  &  &  & rpn0.8/3 & car & 96.4 & 9000\\
 &  &  &  & rpn0.8/4 & car & 96.4 & 9000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RoI-NMS & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $394.7\pm 54.5$ & $3.0\pm 1.0$ & $4003.9\pm 175.6$ &  & car & 97.1 & 12000\\
$22.2\pm 3.5$ & $29.5\pm 5.1$ & $2.0\pm 0.8$ & $3393.1\pm 212.3$ & rpn0.4/1 & car & 97.0 & 12000\\
$22.9\pm 3.8$ & $30.4\pm 5.6$ & $2.9\pm 1.1$ & $3602.1\pm 188.8$ & rpn0.5/1 & car & 97.0 & 12000\\
$25.0\pm 3.8$ & $33.5\pm 5.5$ & $3.0\pm 1.1$ & $3654.0\pm 191.7$ & rpn0.6/1 & car & 97.2 & 12000\\
$28.4\pm 4.3$ & $37.2\pm 6.3$ & $2.9\pm 1.1$ & $3602.3\pm 228.4$ & rpn0.7/1 & car & 97.1 & 12000\\
$30.0\pm 4.8$ & $38.6\pm 6.5$ & $3.0\pm 1.1$ & $3649.0\pm 206.9$ & rpn0.75/1 & car & 97.0 & 12000\\
$29.2\pm 3.8$ & $38.0\pm 5.5$ & $2.9\pm 1.0$ & $3676.3\pm 289.6$ & rpn0.8/1 & car & 96.8 & 12000\\
$32.1\pm 4.3$ & $41.6\pm 6.3$ & $3.0\pm 1.1$ & $3617.0\pm 225.1$ & rpn0.9/1 & car & 96.5 & 12000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RoI-NMS & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $6.1\pm 1.3$ & $0.7\pm 0.2$ & $2338.4\pm 215.6$ &  & human & 79.3 & 1000\\
 &  &  &  & rpn0.6/1 & human & 79.2 & 1000\\
$5.2\pm 0.9$ & $7.7\pm 1.4$ & $1.1\pm 0.4$ & $2564.1\pm 233.4$ & rpn0.7/1 & human & 79.5 & 1000\\
 &  &  &  & rpn0.7/2 & human & 79.3 & 1000\\
$9.2\pm 1.1$ & $10.9\pm 1.3$ & $0.6\pm 0.2$ & $2217.8\pm 214.7$ & rpn0.7/3 & human & 79.2 & 1000\\
$13.2\pm 2.5$ & $15.2\pm 2.9$ & $0.7\pm 0.2$ & $2248.6\pm 305.8$ & rpn0.7/4 & human & 79.2 & 1000\\
$6.2\pm 1.1$ & $8.9\pm 1.6$ & $1.6\pm 0.7$ & $3144.9\pm 271.3$ & rpn0.8/1 & human & 79.5 & 1000\\
 &  &  &  & rpn0.8/2 & human & 79.5 & 1000\\
 &  &  &  & rpn0.8/3 & human & 79.5 & 1000\\
 &  &  &  & rpn0.8/4 & human & 79.5 & 1000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RoI-NMS & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $41.0\pm 8.9$ & $2.5\pm 1.4$ & $3415.5\pm 303.5$ &  & human & 81.6 & 3000\\
 &  &  &  & rpn0.6/1 & human & 81.5 & 3000\\
$11.7\pm 2.1$ & $15.7\pm 2.9$ & $2.7\pm 1.3$ & $3197.3\pm 309.0$ & rpn0.7/1 & human & 81.6 & 3000\\
 &  &  &  & rpn0.7/2 & human & 81.6 & 3000\\
$19.4\pm 2.1$ & $22.2\pm 2.4$ & $2.1\pm 1.2$ & $2973.1\pm 323.9$ & rpn0.7/3 & human & 81.5 & 3000\\
$28.5\pm 5.1$ & $32.0\pm 5.9$ & $2.2\pm 1.3$ & $3269.6\pm 342.9$ & rpn0.7/4 & human & 81.5 & 3000\\
$13.6\pm 2.3$ & $19.1\pm 3.4$ & $2.3\pm 0.9$ & $3294.6\pm 320.2$ & rpn0.8/1 & human & 81.5 & 3000\\
 &  &  &  & rpn0.8/2 & human & 81.6 & 3000\\
 &  &  &  & rpn0.8/3 & human & 81.7 & 3000\\
 &  &  &  & rpn0.8/4 & human & 81.7 & 3000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RoI-NMS & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $141.0\pm 26.9$ & $3.4\pm 2.4$ & $3573.7\pm 321.4$ &  & human & 82.1 & 6000\\
 &  &  &  & rpn0.6/1 & human & 82.0 & 6000\\
$20.8\pm 3.0$ & $27.7\pm 4.2$ & $2.8\pm 1.4$ & $3374.0\pm 269.7$ & rpn0.7/1 & human & 81.8 & 6000\\
 &  &  &  & rpn0.7/2 & human & 82.0 & 6000\\
$32.9\pm 3.5$ & $37.4\pm 4.1$ & $2.9\pm 1.8$ & $2967.2\pm 277.0$ & rpn0.7/3 & human & 82.0 & 6000\\
$45.6\pm 7.1$ & $50.7\pm 8.3$ & $3.2\pm 2.4$ & $3374.9\pm 301.9$ & rpn0.7/4 & human & 82.0 & 6000\\
$24.2\pm 3.9$ & $31.7\pm 5.1$ & $2.3\pm 1.0$ & $3291.1\pm 311.1$ & rpn0.8/1 & human & 81.5 & 6000\\
 &  &  &  & rpn0.8/2 & human & 81.7 & 6000\\
 &  &  &  & rpn0.8/3 & human & 81.8 & 6000\\
 &  &  &  & rpn0.8/4 & human & 81.9 & 6000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RoI-NMS & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $307.9\pm 48.4$ & $3.4\pm 2.1$ & $3643.5\pm 316.2$ &  & human & 82.1 & 9000\\
 &  &  &  & rpn0.4/1 & human & 81.3 & 9000\\
 &  &  &  & rpn0.4/2 & human & 80.5 & 9000\\
 &  &  &  & rpn0.4/3 & human & 80.0 & 9000\\
 &  &  &  & rpn0.4/4 & human & 79.7 & 9000\\
 &  &  &  & rpn0.5/1 & human & 81.7 & 9000\\
 &  &  &  & rpn0.5/2 & human & 81.3 & 9000\\
 &  &  &  & rpn0.5/3 & human & 81.0 & 9000\\
 &  &  &  & rpn0.5/4 & human & 80.8 & 9000\\
 &  &  &  & rpn0.6/1 & human & 82.0 & 9000\\
 &  &  &  & rpn0.6/2 & human & 81.8 & 9000\\
 &  &  &  & rpn0.6/3 & human & 81.9 & 9000\\
$43.4\pm 7.2$ & $49.4\pm 8.4$ & $3.0\pm 2.9$ & $3376.4\pm 292.1$ & rpn0.6/4 & human & 81.8 & 9000\\
$30.2\pm 5.1$ & $38.9\pm 6.6$ & $2.9\pm 1.6$ & $3379.8\pm 307.6$ & rpn0.7/1 & human & 81.8 & 9000\\
$45.6\pm 5.3$ & $53.8\pm 6.7$ & $3.3\pm 2.0$ & $3584.5\pm 459.3$ & rpn0.7/2 & human & 82.0 & 9000\\
$56.4\pm 7.9$ & $64.1\pm 9.4$ & $3.4\pm 2.4$ & $3530.9\pm 473.7$ & rpn0.7/3 & human & 82.0 & 9000\\
$65.3\pm 9.6$ & $73.0\pm 10.9$ & $3.3\pm 2.4$ & $3434.4\pm 269.2$ & rpn0.7/4 & human & 82.1 & 9000\\
$34.8\pm 5.2$ & $44.2\pm 6.8$ & $2.3\pm 1.0$ & $3300.5\pm 287.9$ & rpn0.8/1 & human & 81.5 & 9000\\
 &  &  &  & rpn0.8/2 & human & 81.7 & 9000\\
 &  &  &  & rpn0.8/3 & human & 81.8 & 9000\\
 &  &  &  & rpn0.8/4 & human & 81.9 & 9000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RoI-NMS & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $514.4\pm 66.0$ & $3.3\pm 2.2$ & $3864.9\pm 315.2$ &  & human & 82.1 & 12000\\
$37.6\pm 5.7$ & $47.6\pm 7.5$ & $2.7\pm 1.3$ & $3358.6\pm 310.5$ & rpn0.7/1 & human & 81.8 & 12000\\
 &  &  &  & rpn0.7/2 & human & 82.0 & 12000\\
 &  &  &  & rpn0.7/3 & human & 82.0 & 12000\\
 &  &  &  & rpn0.7/4 & human & 82.1 & 12000\\
$41.5\pm 6.7$ & $52.2\pm 8.9$ & $2.3\pm 1.0$ & $3278.0\pm 235.0$ & rpn0.8/1 & human & 81.5 & 12000\\
 &  &  &  & rpn0.8/2 & human & 81.7 & 12000\\
 &  &  &  & rpn0.8/3 & human & 81.8 & 12000\\
 &  &  &  & rpn0.8/4 & human & 81.9 & 12000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RoI-NMS & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $8.6\pm 1.6$ & $1.4\pm 0.3$ & $2182.3\pm 205.6$ &  & sku & 87.5 & 1000\\
 &  &  &  & rpn0.4/1 & sku & 87.1 & 1000\\
$4.8\pm 0.9$ & $7.2\pm 1.4$ & $1.2\pm 0.2$ & $2085.5\pm 244.4$ & rpn0.5/1 & sku & 88.7 & 1000\\
$13.4\pm 2.4$ & $15.8\pm 2.9$ & $1.4\pm 0.6$ & $2102.6\pm 214.6$ & rpn0.7/3 & sku & 88.5 & 1000\\
$13.2\pm 1.7$ & $14.9\pm 1.9$ & $1.3\pm 0.2$ & $1912.9\pm 217.6$ & rpn0.7/4 & sku & 87.8 & 1000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RoI-NMS & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $61.0\pm 11.6$ & $1.2\pm 0.3$ & $2179.8\pm 277.1$ &  & sku & 90.5 & 3000\\
 &  &  &  & rpn0.4/1 & sku & 90.2 & 3000\\
$10.7\pm 1.8$ & $15.2\pm 2.7$ & $1.2\pm 0.2$ & $2197.8\pm 259.4$ & rpn0.5/1 & sku & 90.4 & 3000\\
$30.2\pm 5.2$ & $34.5\pm 6.1$ & $1.2\pm 0.2$ & $2166.5\pm 250.1$ & rpn0.7/3 & sku & 90.5 & 3000\\
$30.3\pm 3.1$ & $33.6\pm 3.5$ & $1.1\pm 0.2$ & $2029.2\pm 227.1$ & rpn0.7/4 & sku & 90.4 & 3000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RoI-NMS & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $199.9\pm 29.0$ & $1.2\pm 0.2$ & $2272.2\pm 266.7$ &  & sku & 90.5 & 6000\\
 &  &  &  & rpn0.4/1 & sku & 90.2 & 6000\\
$17.0\pm 2.5$ & $22.9\pm 3.6$ & $1.1\pm 0.2$ & $2228.4\pm 270.2$ & rpn0.5/1 & sku & 90.4 & 6000\\
$50.8\pm 8.2$ & $56.6\pm 9.3$ & $1.2\pm 0.2$ & $2179.9\pm 248.3$ & rpn0.7/3 & sku & 90.5 & 6000\\
 &  &  &  & rpn0.7/4 & sku & 90.4 & 6000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RoI-NMS & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $478.4\pm 64.4$ & $1.2\pm 0.2$ & $2599.9\pm 257.2$ &  & sku & 90.5 & 9000\\
 &  &  &  & rpn0.4/1 & sku & 90.2 & 9000\\
 &  &  &  & rpn0.4/2 & sku & 88.6 & 9000\\
 &  &  &  & rpn0.4/3 & sku & 87.3 & 9000\\
 &  &  &  & rpn0.4/4 & sku & 86.5 & 9000\\
$24.7\pm 4.0$ & $32.0\pm 5.4$ & $1.1\pm 0.2$ & $2122.9\pm 283.0$ & rpn0.5/1 & sku & 90.4 & 9000\\
 &  &  &  & rpn0.5/2 & sku & 89.8 & 9000\\
 &  &  &  & rpn0.5/3 & sku & 88.9 & 9000\\
 &  &  &  & rpn0.5/4 & sku & 88.3 & 9000\\
 &  &  &  & rpn0.6/1 & sku & 90.2 & 9000\\
 &  &  &  & rpn0.6/2 & sku & 90.3 & 9000\\
 &  &  &  & rpn0.6/3 & sku & 90.1 & 9000\\
$73.4\pm 9.8$ & $80.0\pm 11.0$ & $1.4\pm 0.4$ & $2022.1\pm 276.2$ & rpn0.6/4 & sku & 89.8 & 9000\\
$32.1\pm 4.2$ & $41.4\pm 5.8$ & $1.0\pm 0.2$ & $2191.5\pm 208.1$ & rpn0.7/1 & sku & 89.8 & 9000\\
$60.9\pm 6.2$ & $69.2\pm 7.4$ & $1.2\pm 0.2$ & $2220.2\pm 253.9$ & rpn0.7/2 & sku & 90.4 & 9000\\
$72.6\pm 10.6$ & $79.9\pm 11.8$ & $1.2\pm 0.3$ & $2250.3\pm 251.4$ & rpn0.7/3 & sku & 90.5 & 9000\\
$94.1\pm 10.5$ & $102.6\pm 11.8$ & $1.2\pm 0.3$ & $2239.9\pm 208.0$ & rpn0.7/4 & sku & 90.5 & 9000\\
 &  &  &  & rpn0.8/1 & sku & 89.1 & 9000\\
 &  &  &  & rpn0.8/2 & sku & 89.6 & 9000\\
 &  &  &  & rpn0.8/3 & sku & 89.9 & 9000\\
 &  &  &  & rpn0.8/4 & sku & 90.0 & 9000\\
\bottomrule
\end{tabular}
\end{table*}\begin{table*}
\centering
\begin{tabular}{cccccccc}
\toprule
RPN-HNMS1 & RPN-NMS & RoI-NMS & Total-Time & approach & data & mAP & prenms\\
\midrule
 & $757.6\pm 75.0$ & $1.3\pm 0.3$ & $2837.9\pm 278.8$ &  & sku & 90.5 & 12000\\
$27.2\pm 4.1$ & $35.2\pm 5.8$ & $1.2\pm 0.2$ & $2142.1\pm 226.7$ & rpn0.4/1 & sku & 90.2 & 12000\\
$29.8\pm 4.5$ & $38.4\pm 6.4$ & $1.1\pm 0.2$ & $2223.5\pm 219.7$ & rpn0.5/1 & sku & 90.4 & 12000\\
 &  &  &  & rpn0.5/2 & sku & 89.9 & 12000\\
$32.1\pm 4.4$ & $40.8\pm 6.0$ & $1.1\pm 0.3$ & $2154.0\pm 203.7$ & rpn0.6/1 & sku & 90.2 & 12000\\
 &  &  &  & rpn0.6/2 & sku & 90.4 & 12000\\
$33.0\pm 4.9$ & $41.1\pm 6.3$ & $1.0\pm 0.2$ & $2056.7\pm 280.2$ & rpn0.7/1 & sku & 89.8 & 12000\\
 &  &  &  & rpn0.7/2 & sku & 90.4 & 12000\\
$88.6\pm 14.0$ & $97.4\pm 15.7$ & $1.2\pm 0.2$ & $2244.4\pm 232.5$ & rpn0.7/3 & sku & 90.5 & 12000\\
 &  &  &  & rpn0.7/4 & sku & 90.5 & 12000\\
 &  &  &  & rpn0.75/2 & sku & 90.1 & 12000\\
 &  &  &  & rpn0.75/3 & sku & 90.3 & 12000\\
 &  &  &  & rpn0.75/4 & sku & 90.4 & 12000\\
$34.6\pm 4.7$ & $43.2\pm 6.2$ & $1.0\pm 0.4$ & $2195.7\pm 181.8$ & rpn0.8/1 & sku & 89.2 & 12000\\
 &  &  &  & rpn0.8/2 & sku & 89.7 & 12000\\
 &  &  &  & rpn0.8/3 & sku & 90.0 & 12000\\
 &  &  &  & rpn0.8/4 & sku & 90.1 & 12000\\
 &  &  &  & rpn0.9/1 & sku & 88.2 & 12000\\
\bottomrule
\end{tabular}
\end{table*}

==> table/rpn1.tex <==
\begin{table}
\centering
\caption{Experiment results with Faster-RCNN-R50-FPN. RPN-NMS and Total represent the time in ms. Speed is for RPN-NMS.}
\label{tbl:rpn}
\begin{tabular}{c}
(a) CARPK \\
\begin{tabular}{c@{~}c@{~}c@{~~}c@{~~}c@{~~}c}
\toprule
 & $K$ & mAP & RPN-NMS & Speed & Total\\
\midrule
NMS &  & 96.9 & $223.3\pm 36.5$ & 1x & $3935.7\pm 184.9$\\
\midrule
\multirow{4}{*}{HNMS} & 1 & \textbf{97.1} & $30.3\pm 5.4$ & \textbf{7.37x} & $3665.6\pm 205.4$\\
 & 2 & \textbf{97.1} & $49.0\pm 6.5$ & \textbf{4.56x} & $3571.5\pm 172.0$\\
 & 3 & 97.0 & $52.3\pm 7.6$ & 4.27x & $3790.5\pm 186.1$\\
 & 4 & 96.9 & $68.8\pm 9.6$ & 3.25x & $3790.6\pm 467.3$\\
\bottomrule
\end{tabular}
\\
\begin{tabular}{ccc@{~~~}ccc@{~~~}ccc}
	\toprule
	\multirow{2}{*}{} & \multirow{2}{*}{$K$} & \multirow{2}{*}{mAP} & \multicolumn{3}{c}{CPU}
	& \multicolumn{3}{c}{GPU} \\
	%	\cline{4-6} \cline{7-9}
	\cmidrule(lr){4-6} \cmidrule(lr){7-9}
	& & & RPN-NMS & Speed & Total & RPN-NMS & Speed & Total \\
	\midrule
	NMS &  & 96.9 & $223.3\pm 36.5$ & 1x & $3935.7$ & $27.2\pm 2.0$ & 1x & $149.0$ \\
	\midrule
	\multirow{4}{*}{HNMS} & 1 & \textbf{97.1} & $30.3\pm 5.4$ & \textbf{7.37x} & $3665.6$ & $9.3\pm 1.2$ & \textbf{2.92x} & $137.9$ \\
	& 2 & \textbf{97.1} & $49.0\pm 6.5$ & \textbf{4.56x} & $3571.5$ & $11.2\pm 1.5$ & 2.43x & $136.9$ \\
	& 3 & 97.0 & $52.3\pm 7.6$ & 4.27x & $3790.5$ & $11.2\pm 1.5$ & 2.43x & $136.9$ \\
	& 4 & 96.9 & $68.8\pm 9.6$ & 3.25x & $3790.6$ & $13.2\pm 1.7$ & 2.06x & $136.2$ \\
	\bottomrule
\end{tabular}

\\
(b) SKU-110K 
\\
\begin{tabular}{c@{~}c@{~}c@{~~}c@{~~}c@{~~}c}
\toprule
 & $K$ & mAP & RPN-NMS & Speed & Total\\
\midrule
NMS &  & \textbf{90.5} & $478.4\pm 64.4$ & \textbf{1x} & $2599.9\pm 257.2$\\
\midrule
\multirow{4}{*}{HNMS} & 1 & 89.8 & $41.4\pm 5.8$ & 11.56x & $2191.5\pm 208.1$\\
 & 2 & 90.4 & $69.2\pm 7.4$ & 6.91x & $2220.2\pm 253.9$\\
 & 3 & \textbf{90.5} & $79.9\pm 11.8$ & \textbf{5.99x} & $2250.3\pm 251.4$\\
 & 4 & \textbf{90.5} & $102.6\pm 11.8$ & \textbf{4.66x} & $2239.9\pm 208.0$\\
\bottomrule
\end{tabular}
\\
(c) CrowdHuman
\\
\begin{tabular}{c@{~}c@{~}c@{~~}c@{~~}c@{~~}c}
\toprule
 & $K$ & mAP & RPN-NMS & Speed & Total\\
\midrule
NMS &  & \textbf{82.1} & $307.9\pm 48.4$ & \textbf{1x} & $3643.5\pm 316.2$\\
\midrule
\multirow{4}{*}{HNMS} & 1 & 81.8 & $38.9\pm 6.6$ & 7.92x & $3379.8\pm 307.6$\\
 & 2 & 82.0 & $53.8\pm 6.7$ & 5.72x & $3584.5\pm 459.3$\\
 & 3 & 82.0 & $64.1\pm 9.4$ & 4.80x & $3530.9\pm 473.7$\\
 & 4 & \textbf{82.1} & $73.0\pm 10.9$ & \textbf{4.22x} & $3434.4\pm 269.2$\\
\bottomrule
\end{tabular}

\end{tabular}

\end{table}

==> table/soft_retina_table.tex <==
\begin{table}
\centering
\caption{Experiment results on CARPK with Retina-R50-FPN. The columns of HNMS, NMS and Total represent the time cost in ms. Speed is for the total cost by HNMS and NMS.}
\label{tbl:retina_CARPK}
\begin{tabular}{c@{~}c@{~}c@{~~}c@{~~}c@{~~}c@{~~}c}
\toprule
 & $K$ & mAP & HNMS & NMS & Speed & Total\\
\midrule
NMS &  & 95.3 &  & $40710.5\pm 4402.8$ & 1x & $42980.8\pm 6686.9$\\
\midrule
\multirow{4}{*}{HNMS} & 1 & 95.3 & $22.6\pm 5.4$ & $10160.4\pm 2582.2$ & 4.00x & $11878.1\pm 2591.7$\\
 & 2 & \textbf{95.4} & $31.8\pm 6.3$ & $7210.5\pm 1925.8$ & \textbf{5.62x} & $8901.7\pm 1939.2$\\
 & 3 & \textbf{95.4} & $39.5\pm 8.1$ & $5451.7\pm 1565.6$ & \textbf{7.41x} & $7133.3\pm 1573.8$\\
 & 4 & \textbf{95.4} & $49.4\pm 11.2$ & $4701.4\pm 1372.1$ & \textbf{8.57x} & $6415.1\pm 1402.6$\\
\bottomrule
\end{tabular}
\end{table}\begin{table}
\centering
\caption{Experiment results on SKU-110K with Retina-R50-FPN. The columns of HNMS, NMS and Total represent the time cost in ms. Speed is for the total cost by HNMS and NMS.}
\label{tbl:retina_SKU-110K}
\begin{tabular}{c@{~}c@{~}c@{~~}c@{~~}c@{~~}c@{~~}c}
\toprule
 & $K$ & mAP & HNMS & NMS & Speed & Total\\
\midrule
NMS &  & 91.9 &  & $37673.2\pm 2564.3$ & 1x & $39260.5\pm 2692.3$\\
\midrule
\multirow{4}{*}{HNMS} & 1 & 91.9 & $21.8\pm 3.5$ & $11042.8\pm 1837.5$ & 3.40x & $12639.3\pm 1877.0$\\
 & 2 & \textbf{92.0} & $30.3\pm 5.5$ & $6902.1\pm 1144.8$ & \textbf{5.43x} & $8434.5\pm 1214.3$\\
 & 3 & \textbf{92.0} & $38.1\pm 6.5$ & $5524.2\pm 943.4$ & \textbf{6.77x} & $7038.9\pm 1011.7$\\
 & 4 & \textbf{92.0} & $45.5\pm 7.0$ & $4697.9\pm 899.0$ & \textbf{7.94x} & $6258.0\pm 988.1$\\
\bottomrule
\end{tabular}
\end{table}\begin{table}
\centering
\caption{Experiment results on CrowdHuman with Retina-R50-FPN. The columns of HNMS, NMS and Total represent the time cost in ms. Speed is for the total cost by HNMS and NMS.}
\label{tbl:retina_CrowdHuman}
\begin{tabular}{c@{~}c@{~}c@{~~}c@{~~}c@{~~}c@{~~}c}
\toprule
 & $K$ & mAP & HNMS & NMS & Speed & Total\\
\midrule
NMS &  & \textbf{78.6} &  & $44272.1\pm 3350.4$ & \textbf{1x} & $45821.6\pm 3418.3$\\
\midrule
\multirow{4}{*}{HNMS} & 1 & \textbf{78.6} & $26.7\pm 6.8$ & $17549.4\pm 2625.1$ & \textbf{2.52x} & $19295.2\pm 2706.6$\\
 & 2 & \textbf{78.6} & $39.0\pm 7.4$ & $11474.2\pm 2039.7$ & \textbf{3.85x} & $13125.2\pm 2053.0$\\
 & 3 & \textbf{78.6} & $51.5\pm 8.8$ & $9234.0\pm 1838.6$ & \textbf{4.77x} & $10937.6\pm 1863.9$\\
 & 4 & \textbf{78.6} & $65.7\pm 35.9$ & $7940.9\pm 1713.3$ & \textbf{5.53x} & $9717.2\pm 1791.1$\\
\bottomrule
\end{tabular}
\end{table}
